Less is More: Revisiting the Gaussian Mechanism for Differential Privacy

Differential privacy via output perturbation has been a de facto standard for releasing query or computation results on sensitive data. However, we identify that all existing Gaussian mechanisms suffer from the curse of full-rank covariance matrices. To lift this curse, we design a Rank-1 Singular Multivariate Gaussian (R1SMG) mechanism. It achieves DP on high dimension query results by perturbing the results with noise following a singular multivariate Gaussian distribution, whose covariance matrix is a randomly generated rank-1 positive semi-definite matrix. In contrast, the classic Gaussian mechanism and its variants all consider deterministic full-rank covariance matrices. Our idea is motivated by a clue from Dwork et al.'s seminal work on the classic Gaussian mechanism that has been ignored in the literature: when projecting multivariate Gaussian noise with a full-rank covariance matrix onto a set of orthonormal basis, only the coefficient of a single basis can contribute to the privacy guarantee. This paper makes the following technical contributions. The R1SMG mechanisms achieves DP guarantee on high dimension query results, while its expected accuracy loss is lower bounded by a term that is on a lower order of magnitude by at least the dimension of query results compared existing Gaussian mechanisms. Compared with other mechanisms, the R1SMG mechanism is more stable and less likely to generate noise with large magnitude that overwhelms the query results, because the kurtosis and skewness of the nondeterministic accuracy loss introduced by this mechanism is larger than that introduced by other mechanisms.

==> sections/intuitive.tex <==



\section{The Intuition behind R1SMG}\label{sec:explain-property}


As introduced in Section \ref{sec:contribution}, the expected accuracy loss of R1SMG is  lower bounded by  $C_R(\Delta_2 f)^2$ where $C_R = \frac{2}{\epsilon \psi}$ has a decreasing trend as $M$ increases, and converges to $\frac{2}{\epsilon}$ as $M$ approaches infinity (Theorem \ref{theorem:r1smg_asymptotic}).  Thus, we have the following property (see Property \ref{claim:magic_claim}) that is   missing in all existing DP mechanisms. Here, we provide an intuitive explanation on it. {\color{blue}In  Section \ref{sec:discussion_r1smg},  we will formally prove the expected accuracy loss of R1SMG.}



\begin{property}%\textbf{(Informal)}%\textbf{Unique Property of R1SMG (Informal).}
\label{claim:magic_claim}
 For any fixed   $\epsilon$, $\delta$, and $\Delta_2f$ the magnitude of the noise required  to attain $(\epsilon,\delta)$-DP on $f(\bm{x})\in\R^M$   can have a non-increasing trend regarding $M$. For sufficiently large $M$, the magnitude of the noise can converge to  a constant. 
\end{property}


Due to the widely accepted common practice of perturbing each component of $f(\bm{x})$ using i.i.d. Gaussian noise to achieve DP, it makes sense that   larger dimensional    $f(\bm{x})$ requires larger magnitude of noises. Thus, Property \ref{claim:magic_claim} is counterintuitive and 
seems to be a ``magic''. Yet, it can be intuitively explained as follows. Given a database $\bm{x}$ represented as histogram, we consider a {\color{blue}normalized} counting query function $f(\bm{x}) = \frac{1}{M}Q\bm{x} \in \R^M$, where $Q$ is a binary matrix.   A higher dimension of $f(\bm{x})$ means a larger number of queries applied to the same dataset $\bm{x}$. Subsequently, the chances that the query results become dependent with each other increases as the query number increases. For instance, suppose that the $i$th and $j$th query, i.e., $f(\bm{x})_i$ and $f(\bm{x})_j$ are dependent, {\color{blue}particularly, $f(\bm{x})_j$ can be fully determined by $f(\bm{x})_i$}. Then,   the privacy leakage on $\bm{x}$ by observing $f(\bm{x})_i$,  $f(\bm{x})_j$, or $[f(\bm{x})_i\ f(\bm{x})_j]$ would be identical. Hence, intuitively, no more noise is needed to perturb  $[f(\bm{x})_i\ f(\bm{x})_j]$ than that for perturbing $f(\bm{x})_i$. It implies that as $M$ increases and the queried results become dependent, it is possible to achieve DP by perturbing $f(\bm{x})$ using noise of a non-increasing magnitude. %In what follows, we provide an informal technical reasoning for the above example. 
Moreover, when $M$ becomes sufficiently large such that the query vectors (rows in $Q$) are linearly dependent, by observing $f(\bm{x})$ or the set of independent query vectors, the privacy leakage of $\bm{x}$ is identical. Therefore, the same amount of noises can be used to sanitize both (refer to \cite{sun2019relationship} for an analysis from the perspective of mutual information). Thus,   for sufficiently large $M$, the magnitude of the noise can converge to a constant.

% \textbf{An informal reasoning.} We consider $f(\cdot)$ as {\color{blue}normalized} count queries as an example. Given a database $\bm{x}$ represented as histogram, a set of $M$ counting queries can be represented as a binary matrix $Q\in\{0,1\}^{M\times |\bm{x}|}$. Then, $f(\bm{x}) = \frac{1}{M} Q\bm{x}\in\R^M$ is the query results. For simplicity, we assume that each element of $Q$ has an equal probability of being 0 or 1. If $M> |\bm{x}|$,   the query vectors (rows in $Q$) are linearly dependent, i.e.,  given $|\bm{x}|$ independent query results, the other $M-|\mathcal{X}|$ results can be determined. In other words, by observing $f(\bm{x})$ or the set of  $|\mathcal{X}|$ independent query, the privacy leakage of $\bm{x}$ are identical. Thus, the same amount of noises can be used to sanitize both (refer to \cite{sun2019relationship} for an analysis from the perspective of mutual information). Thus, noise of a  constant magnitude can  protect the privacy of $f(\bm{x})$ for sufficiently large $M$, e.g., $M\geq |\bm{x}|$.

% Now we consider the case where $M\leq |\mathcal{X}|$. Suppose that $Q$ has $M_1$ independent rows, then the space spanned by $Q$ has dimension $M_1$ (i.e., $rank(Q)=M_1\leq|\mathcal{X}|$). Adding a new row to $Q$   leaves the rank unchanged with probability $2^{M_1-|\mathcal{X}|}$  \cite[p. 127]{kolchin1999random}). In other words, rows in $Q$ becomes linear dependent with probability $2^{M_1-|\mathcal{X}|}$. When $M_1$ increases from 1 to $|\mathcal{X}|$, the probability of $Q$ becomes rank deficiency also increases.  This implies that  there is an increasing probability that a higher dimensional $f(\bm{x})$ will lead to the same amount of privacy leakage compared with a lower dimensional $f(\bm{x})$. 


% {\color{blue}The above informal reasoning suggests that it is feasible to use noise with non-increasing magnitude to sanitize higher dimensional $f(\bm{x})$. In  Section \ref{sec:discussion_r1smg}, we will rigorously prove that the noise magnitude has a decreasing trend as $M$ increases.}

% Combing the non-increasing privacy leakage as $M$ increases and constant privacy leakage when $M$ is sufficiently large. It essentially suggests that less amount of noise can sanitize higher dimensional query results, when $M$ goes to infinity, the magnitude of the noise should be a constant. We   rigorously  prove this in  Section \ref{sec:discussion_r1smg}.



==> sections/main_tech_backup.tex <==





\section{Lifting the Curse}\label{sec:redfrog}
% of Full Rank Covariance Matrices
% Motivated by the results in the previous section, i.e., the expected accuracy loss  equals   the trace of the full rank covariance matrices of the   noises. 
% % depends on the degrees of freedom in the additive Gaussian noises, 
% Now, we  present the developed %the rank 1 singular multivariate Gaussian mechanism, i.e., 
% R$1$SMG, which improves the differentially private  high dimensional   query by constructing random-rank-1 positive semi-definite covariance matrices. %This section  gives an affirmative answer to $\mathbf{Q}1$. 
% when perturbing the matrix-valued query result $f(D)$. 


In what follows, we    present the developed R$1$SMG mechanism, which lifts the identified curse of full rank covariance matrices. In particular, we first introduce its noise generation process and   a sufficient condition for it to achieve  $(\epsilon,\delta)$-DP. %Then, we present the detailed proof of the proposed condition. 
Next, we analyze the asymptotic behavior of R1SMG as $M$ increases, 
discuss the privacy leakage of utilizing   vector in the null space of the noise, and describe the implementation process of R1SMG.  %Finally, we graphically compare the noises generated by   R1SMG and other mechanisms.


% which perturbs the matrix-valued query result $f(D)$ using noises attributed to a singular multivariate Gaussian distribution with a rank $r$ covariance matrix. Then, we study the differential privacy guarantee of $r$SMGM. Next, we consider $r=1$ and present R$1$SMG, which provides the highest query accuracy in the $r$SMGM family. 


\subsection{R$1$SMG: Multivariate Gaussian Noises  Using  Random-Rank-1 Covariance Matrix}\label{sec:rsmgm}
%Before formally introducing  R$1$SMG, 
We first provide the statistical background on the singular multivariate Gaussian distribution with a given rank $r$ covariance matrix, e.g., $\bm{\Pi}$ and $Rank(\bm{\Pi})=r$. 
% In general, a multivariate Gaussian distribution with a singular covariance matrix of rank $r$ is defined as follows.
\begin{definition}\textbf{Singular Multivariate Gaussian Distribution \cite{khatri1968some,cramer1999mathematical,rao1973linear,srivastava2009introduction}.} 
A  $M$-dimensional   random variable $\mathbf{x} = [x_1,x_2,\cdots,x_{M}]^T$ has a singular multivariate Gaussian distribution with mean $\mathbf{\mu}\in\mathbb{R}^{M}$ and singular covariance matrix $\bm{\Pi}\in\mathbb{PSD}^{M\times M}$ with rank $r$, i.e., $\mathbf{x}\sim\mathcal{N}(\mathbf{\mu},\bm{\Pi})$ and $Rank(\bm{\Pi})=r<M$, if its  PDF is 
% \begin{small}
\begin{equation*}
f_{\mathbf{x};Rank(\bm{\Pi})=r}=\frac{(2\pi)^{-r/2}    \exp\big(-\frac{1}{2}  (\mathbf{x}-\mathbf{\mu})^T \bm{\Pi}^{\dagger} (\mathbf{x}-\mathbf{\mu})\big)       }{\sqrt{\sigma_1(\bm{\Pi}) \cdots\sigma_r(\bm{\Pi})}},
\label{singular_pdf}
\end{equation*}
% \end{small}
where $\sigma_i(\bm{\Pi})$ is the $i$-th nonzero singular value of $\bm{\Pi}$, and $\bm{\Pi}^{\dagger}$ is the generalized inverse of $\bm{\Pi}$.   $\bm{\Pi}^{\dagger} = \mathbf{V}_r\bm{\Lambda}_r^{-1}\mathbf{V}_r^T$, $\bm{\Lambda}_r = \text{diag}(\sigma_1(\bm{\Pi}), \cdots,\sigma_r(\bm{\Pi}))\in\R^{r\times r}$, and $\mathbf{V}_r\in\R^{M\times r}$ is the matrix of singular vectors corresponding to the $r$ nonzero singular values.
\label{def:singular_pdf}
\end{definition}


% \begin{remark}
% Singular multivariate Gaussian distribution has been widely adopted in modelling the distribution of residual in multivariate linear regression \cite{rao1973linear}, statistical quality control \cite{genz2000numerical},  and sampling size determination \cite{kwong1996singular}. It is an example of   the \textbf{pure singular distribution}, which describes the probability mass concentrated on the  set of  Lebesgue measure zero.\footnote{
% According to the Lebesgue decomposition theorem (p.140   \cite{feller1957introduction}, p.71 \cite{McCord1964introduction}, \cite{hewitt2013real,koopmans1983teaching,koopmans1969some}), the distribution   function ($F$) of a random variable $\x$ can be decomposed as 
% \begin{equation*}
%     F = \alpha F_d + \beta F_{ac} + \gamma F_{s},\ \     \alpha+\beta+\gamma=1,
% \end{equation*}
% where $F_d$ is the pure discrete component that can be completely determined by the probability mass function, $F_{ac}$ is the pure absolutely continuous component which is completely determined by the probability density function, and $F_s$ is the singular component describing  the probability mass supported on Lebesgue measure zero sets. One of the most well-known singular distributions is the Cantor distribution which has support on the Cantor set   \cite{hewitt2013real}.} %created by iterative deleting the open middle third from the set of line segments, i.e., $\mathcal{C} = \cap_{n=1}^{\infty}C_n$, where $C_n = $}
% \end{remark}

% Recall that 
% It is noteworthy that (\ref{singular_pdf})




Samples of  $f_{\mathbf{x};Rank(\bm{\Pi})=r}$ (e.g., $\mathbf{n}$) can be generated by applying the disintegration theorem \cite{fremlin2000measure}. In particular, if $\mathbf{\mu}=\mathbf{0}$, by defining a linear mapping %$\mathbf{n} = \mathbf{V}_r\bm{\Lambda}_r^{1/2}\mathbf{z}$,  
\begin{equation}
\mathbf{n} = \mathbf{V}_r\bm{\Lambda}_r^{1/2}\mathbf{z},\quad \mathrm{and}\quad \mathbf{z}\sim\mathcal{N}(\mathbf{0},\mathbf{I}_{r\times r}),
\label{mapping_singular}
\end{equation}
where $\bm{\Lambda}_r^{1/2} = \text{diag}(\sqrt{\sigma_1(\bm{\Pi})},\sqrt{\sigma_2(\bm{\Pi})},\cdots,\sqrt{\sigma_r(\bm{\Pi})})\in\R^{r\times r}$, 
% and  $\mathcal{N}(\mathbf{0},\mathbf{I}_{r\times r})$ stands for the multivariate Gaussian distribution with zero mean and standard covariacne matrix $\mathbf{I}_{r\times r}$, 
then $\mathbf{n}$ is attributed to a singular multivariate Gaussian distribution with a rank $r$ covariance matrix.  
This can easily be verified by checking   the covariance matrix of $\mathbf{n}$; % i.e.,  of the generated noise sample $\mathbf{n}$, i.e., 
 \begin{equation}\label{eq:emp-covariance}
 \begin{aligned}
     Cov(\mathbf{n}) = & Cov(\mathbf{V}_r\bm{\Lambda}_r^{1/2}\mathbf{z})
 = \mathbf{V}_r\bm{\Lambda}_r^{1/2} Cov(\mathbf{z})(\mathbf{V}_r\bm{\Lambda}_r^{1/2})^T\\
\stackrel{(*)}= & \mathbf{V}_r\bm{\Lambda}_r^{1/2} \mathbf{I}_{r\times r}(\mathbf{V}_r\bm{\Lambda}_r^{1/2})^T = \mathbf{V}_r \bm{\Lambda}_r \mathbf{V}_r^T  = \bm{\Pi}
 \end{aligned},
 \end{equation}
where $(*)$ is due to  $\mathbf{z}\sim\mathcal{N}(\mathbf{0},\mathbf{I}_{r\times r})$. Then clearly, $Cov(\mathbf{n})=r$.

% we have $\mathbf{V}_r \bm{\Lambda}_r \mathbf{V}_r^T  = \bm{\Pi}$, which is a rank $r$ singular matrix. 
 
% is indeed the desired singular covariance matrix of rank $r$, where $*$ is because $\mathbf{z}\sim\mathcal{N}(\mathbf{0},\mathbf{I}_{r\times r})$.


When $r=1$, the singular covariance matrix $\bm{\Pi}$ only has 1 non-zero singular value, and we denote it as $\sigma_{*}$. As a result, (\ref{mapping_singular}) becomes
    \vspace{-2mm}
\begin{equation}
\mathbf{n} = \mathbf{v}\sqrt{\sigma_*}z,\quad \mathrm{and}\quad z\sim\mathcal{N}(0,1),\quad \mathbf{v}^T\mathbf{v} = 1.
\label{mapping_singular_rank1}
\end{equation}
% To avoid confusing, we would like to highlight that, following the notation convention in Definition \ref{singular_pdf},  $\sigma_*$ denotes the singular value of  $\bm{\Pi}$.  Whereas $\sigma$ (or $\sigma_A$) denotes the standard deviation of noise used in the classical Gaussian (or analytic Gaussian) mechanism. 








\textbf{Singular multivariate Gaussian distribution with a random-rank-1 covariance matrix.} It is noteworthy that in (\ref{mapping_singular_rank1}), $\mathbf{v}$ needs to be generated randomly to thwart  attacks which takes advantage  of sensing vectors in the null space of $\mathbf{v}$ (or $\mathbf{n}$). In Section \ref{sec:null_space_attack}, we will show that by sampling $\mathbf{v}$ uniformly at random, such attacks will success with \textbf{zero probability}. 

Since $\mathbf{v}$ is an   orthonormal vector of dimension $M\times 1$, one common approach to generate $\mathbf{v}$ randomly is by uniformly sampling from a specific  Stiefel manifold, i.e., $\mathbb{V}_{1,M} = \{\mathbf{v}\in\R^{M\times 1}:\mathbf{v}^T\mathbf{v} = 1\}$, which represents  the unite sphere $\mathbb{S}^{M-1}$  embedded in $\R^{M}$. In Statistics literature, the PDF of the \emph{uniform distribution on the Stiefel manifold $\mathbb{V}_{1,M}$}  is given by 
\begin{equation}\label{eq:stiefel_uniform}
    f(\mathbf{v}) = \frac{1}{\mathrm{Vol}(\mathbb{V}_{1,M})}, \quad \forall \mathbf{v} \in \mathbb{V}_{1,M},
\end{equation}
(see, e.g.,  \cite{gupta2018matrix}  page 280, equation 8.2.2,  \cite{camano2006statistics} page 17, and  \cite{chikuse2012statistics} page 30 which  gives the characteristic  function of  (\ref{eq:stiefel_uniform})).  In particular, the constant  $\mathrm{Vol}(\mathbb{V}_{1,M}) = \frac{2 \pi^{M /2}}{\Gamma(M/2)}$ (see \cite{gupta2018matrix} page 19 and 26) is the total volume  of $\mathbb{V}_{1,M}$ and $\Gamma(\cdot)$ is the ordinary gamma function    \cite{gupta2018matrix}.\footnote{{\color{black}This  result can be easily obtained by setting $p=1$ in Theorem 1.4.9 on page 25 of  \cite{gupta2018matrix}. The physical meaning of $\mathrm{Vol}(\mathbb{V}_{1,M})$ can be interpreted by draw an analogy with an uniform distribution on 1D Euclidean space, i.e.,   uniform distribution on interval $[a,b]$ has PDF $f(x) = \frac{1}{b-a}$, and $b-a$ is the total length (i.e., measure) of  $[a,b]$. Technically speaking,  $\mathrm{Vol}(\mathbb{V}_{1,M})$ plays the same role on $\mathbb{V}_{1,M}$ that the Lebesgue measure plays in   Euclidean space \cite{camano2006statistics}. In the special cases, when $M=3$, $\mathrm{Vol}(\mathcal{V}_{1,3}) = 4\pi$ is the surface area of an unit sphere in 3D space, and when $M=2$, $\mathrm{Vol}(\mathcal{V}_{1,2}) = 2\pi$ is the circumference  of an unit 
circle  in 2D space.}} 

We use $\mathbf{v}\sim\mathcal{U}(\mathbb{V}_{1,M})$ to represent that $\mathbf{v}$ is a random variable uniformly sampled from $\mathbb{V}_{1,M}$. As a consequence, the linear mapping defined in (\ref{mapping_singular_rank1}) becomes
\begin{equation}
\begin{aligned}
\mathbf{n} = \mathbf{v}\sqrt{\sigma_*}z,\quad 
\text{where}\quad  z\sim\mathcal{N}(0,1),\quad \mathbf{v}\sim\mathcal{U}(\mathbb{V}_{1,M}).
\end{aligned}
\label{mapping2}
\end{equation}






% \subsubsection{Singular multivariate Gaussian distribution with a random rank $r$ covariance matrix}

Now, we introduce the  proposed R$1$SMG   and provide a sufficient condition for it to achieve differential privacy. %  in Theorem \ref{thm_multivariate}.
\begin{definition}\textbf{The Proposed R$1$SMG.} Given a high dimensional  query $f(\bm{x})\in\R^{M}$,   R$1$SMG is defined as 
    \vspace{-2mm}
\begin{equation*}
    \mathcal{M}_{R1SMG}\Big(f(\bm{x})\Big)  = f(\bm{x})+ \mathbf{n},
\end{equation*}
where   $\mathbf{n}$ (generated via (\ref{mapping2})) is the noise attributed to a singular multivariate Gaussian distribution with a random-rank-$1$ covaraince matrix.
% $\mathbf{n}\sim\mathcal{N}(\mathbf{0},\bm{\Pi})$, $\bm{\Pi}\in\mathbb{PSD}^{MN\times MN}$,   $Rank(\bm{\Pi})=r$, 
% and ${\rm{resize}}(\cdot, N, M)$ is an operator that resizes $\mathbf{n}\in\R^{MN\times 1}$ into an $N\times M$ matrix.\footnote{For example, ${\rm{resize}}([1,2,3,4,5,6]^T,2,3) = \begin{bmatrix}
% 1 & 3 & 5\\
% 2 & 4 & 6
% \end{bmatrix}$.}
\label{def:rsmgm}
\end{definition}











The next theorem presents a sufficient condition on $\sigma_*$ in (\ref{mapping2}) for  R$1$SMG to achieve differential privacy.





%\begin{theorem}
% R$1$SMG achieves $\big(\epsilon,\delta_1+\delta_2-\delta_1\delta_2\big)$-differential privacy, $\forall \delta_1, \delta_2\in(0,1)$, if $\sigma_{*} \geq  \frac{\Delta_2f^2 \omega}{\epsilon^2 \psi}$, 
% % \begin{equation*}
% % \sigma_{*} \geq  \frac{\Delta_2f^2 \omega}{\epsilon^2 \psi}, 
% % \label{suff_cond1}
% % \end{equation*}
% where   $\omega$ and $\psi$ are %given by
% \begin{gather*}
%     \begin{aligned}
%     \omega = 2\Big( 2\sqrt{- \ln\delta_1}-2\ln\delta_1+1\Big),\qquad \psi = \left(\frac{\delta_2\Gamma(\frac{MN-1}{2})}{\sqrt{\pi}\Gamma(\frac{MN}{2})}\right)^{\frac{2}{MN-2}},
%     \end{aligned}
% \end{gather*}
% and   $\Gamma(\cdot)$ is Gamma  function.
% % $\sigma_{r}$ is the $r$-th largest diagonal value  (i.e., the smallest nonzero diagonal value)  of $\bm{\Lambda}_r$, and $\omega(\delta,r) = 2\sqrt{-r\ln \delta}-2\ln \delta+r$.
% \label{thm_multivariate}
% \end{theorem}



\begin{theorem}\label{thm_multivariate}
R$1$SMG achieves $(\epsilon,\delta)$-DP,  if $\sigma_{*} \geq  \frac{2(\Delta_2f)^2}{\epsilon \psi}$, 
% \begin{equation*}
% \sigma_{*} \geq  \frac{\Delta_2f^2 \omega}{\epsilon^2 \psi}, 
% \label{suff_cond1}
% \end{equation*}
where   $\psi = \left(\frac{\delta\Gamma(\frac{M-1}{2})}{\sqrt{\pi}\Gamma(\frac{M}{2})}\right)^{\frac{2}{M-2}}$, 
and   $\Gamma(\cdot)$ is Gamma  function.
\end{theorem}
\begin{proof}First, we review the following lemmas which are important to the proof.
\begin{lemma}\textbf{Distribution  of Angle between Random Points on Unit Sphere (see page 1845 and 1860   of \cite{cai2013distributions}).} Let $h$ and $g$ be two randomly selected  points on   unit sphere $\mathbb{S}^{P-1}$ (embedded in $\R^P$). Let $\mathbf{h}$ (resp. $\mathbf{g}$) be the vector connecting the center of the sphere and $h$ (resp. $g$). $\theta$ denotes the angle ($\theta\in[0, \pi]$) between $\mathbf{h}$ and $\mathbf{g}$. Then%\footnote{The closed-from expression is shown on page 25 of \cite{cai2013distributions}} 
\begin{equation}
    \Pr\left[\left|\theta-\frac{\pi}{2}\right|\geq \theta_0\right] \leq \sqrt{\pi}\frac{\Gamma(\frac{P}{2})}{\Gamma(\frac{P-1}{2})} cos(\theta_0)^{P-2},
\end{equation}
where $\theta_0$ is a given radian and $0\leq \theta_0\leq\frac{\pi}{2}$. 
\label{lemma:angle}
\end{lemma}


% Now, we start the proof by analyzing 


Then, inspired by Dwork et al.'s work~\cite{dwork2014algorithmic} (reviewed in Section \ref{sec:evidence}), we  investigate the PRLM associated with our developed R1SMG. 
% the alternative definition of $(\epsilon,\delta)$-DP (discussed in Section \ref{sec:pre}). Let $\bm{x}$ and $\bm{x}'$ be a pair of neighboring datasets. 
Assume that $\mathbf{n}$ and $\mathbf{n}'$ are the random noises used to perturb $f(\bm{x})$ and $f(\bm{x}')$, respectively.  Then, R1SMG achieves $(\epsilon,\delta)$-DP if %the corresponding  privacy loss random variable (denoted as  
$\mathrm{PLRV}^{(\mathbf{s})}_{(R1SMG(\bm{x})||R1SMG(\bm{x}'))}$  is upper bounded by    $\epsilon$ with probability at least $1-\delta$, i.e., 
\begin{equation}\label{eq:plrv-r1smg}
\mathrm{PLRV}^{(\mathbf{s})}_{(R1SMG(\bm{x})||R1SMG(\bm{x}'))}= \ln\left(\frac{\Pr[f(\bm{x})+\mathbf{n} = \mathbf{s}]}{\Pr[f(\bm{x}')+\mathbf{n}'= \mathbf{s}]}\right) \leq \epsilon,
\end{equation}
hold probability at least $1-\delta$.




According to (\ref{mapping2}), without loss of generality, let 
\begin{equation}\label{eq:noise_neighbor}
    \mathbf{n} = \sqrt{\sigma_*} z_1\mathbf{h},\quad
    \mathbf{n}' =  \sqrt{\sigma_*} z_2 \mathbf{g},
\end{equation}
% $\mathbf{n} = \sqrt{\sigma_*} z_1\mathbf{h} $ and $\mathbf{n}' =  \sqrt{\sigma_*} z_2 \mathbf{g}$,
where   $z_1, z_2\sim\mathcal{N}(0,1)$ and $\mathbf{h},\mathbf{g}\sim\mathcal{U}(\mathbb{V}_{1,M})$. %Then, we can  immediate  have %the following relationships
% obtain  the squared norm of the additive noise, e.g., $\mathbf{n}'$, as 
% \begin{equation*}
%     ||\mathbf{n}'||_2^2 = (\sqrt{\sigma_*} z_2 \mathbf{g})^T\sqrt{\sigma_*} z_2 \mathbf{g} \stackrel{*}=   \sigma_*  z_2^2,
% \end{equation*}
% where $*$ is because $\mathbf{g}\in\mathbb{V}_{1,M}$, thus $\mathbf{g}^T\mathbf{g} =1$.
% \begin{equation}\label{eq:mapping_back01}
%     % \begin{aligned}
%     z_1 = \sigma_*^{-1/2}\mathbf{h}^T\mathbf{n},\quad
%     z_2 = \sigma_*^{-1/2}\mathbf{g}^T\mathbf{n}'.
%     % \end{aligned}
% \end{equation}






% For neighboring datasets $\bm{x}$ and $\bm{x}'$,  our proposed R1SMG considers the following sample space
$\mathrm{PLRV}^{(\mathbf{s})}_{(R1SMG(\bm{x})||R1SMG(\bm{x}'))}$   in (\ref{eq:plrv-r1smg}) involves four random variables (i.e., $z_1$, $z_2$, $\mathbf{h}$, and $\mathbf{g}$). It considers the   log-ratio of the probability densities $\Pr[f(\bm{x})+\mathbf{n} = \mathbf{s}]$ and $\Pr[f(\bm{x}')+\mathbf{n}'= \mathbf{s}]$. Thus, it implies the following   sampling space     $\mathcal{T}$, which is a subspace of the universe $\Omega$, i.e., 
\begin{equation*} 
\begin{aligned}
\mathcal{T} = &\Big\{z_1, z_2, \mathbf{h}, \mathbf{g}: z_1, z_2\sim \mathcal{N}(0,1),  \mathbf{h}, \mathbf{g}\sim \mathcal{U}(\mathbb{V}_{1,M}), \\
& f(\bm{x})+\sqrt{\sigma_*}z_1\mathbf{h} = \mathbf{s}\in \mathcal{S}, f(\bm{x}')+\sqrt{\sigma_*}z_2\mathbf{g} = \mathbf{s}\in \mathcal{S}\Big\}\\
\subset & \Omega = \Big\{z_1, z_2, \mathbf{h}, \mathbf{g}: z_1, z_2\sim \mathcal{N}(0,1),  \mathbf{h}, \mathbf{g}\sim \mathcal{U}(\mathbb{V}_{1,M})\Big\},
\end{aligned}
\end{equation*}
where $\mathcal{S}$ denotes all possible outcome of R1SMG. 





% the sampling space associated with it is
% \begin{equation*}
%     \mathcal{T}=\{z_1, z_2, \mathbf{h}, \mathbf{g}: z_1, z_2\sim \mathcal{N}(0,1), \mathbf{h}, \mathbf{g}\sim \mathcal{U}(\mathbb{V}_{1,M}) \}.
% \end{equation*}

Let $\theta\in[0,\pi]$ be the angle between $\mathbf{h}$ and $\mathbf{g}$. We define  an  event  $\mathcal{A}$ which is also a subspace of the universe $\Omega$.  
% involving four random variables ($z_1$, $z_2$, $\mathbf{h}$, and $\mathbf{g}$) % (which is a subspace of $\mathcal{T}$, i.e., $\mathcal{A}\subset \mathcal{T}$)  
\begin{equation*}\label{eq:the_set}
    \resizebox{1.05\linewidth}{!}{$\mathcal{A} = \left\{z_1, z_2, \mathbf{h}, \mathbf{g}: z_1, z_2\sim \mathcal{N}(0,1),  \mathbf{h}, \mathbf{g}\sim \mathcal{U}(\mathbb{V}_{1,M}),  \left|\theta-\frac{\pi}{2}\right| < \theta_0\right\},$}
\end{equation*}
where $\theta_0 = arccos\left(\left(\frac{\delta\Gamma(\frac{M-1}{2})}{\sqrt{\pi}\Gamma(\frac{M}{2})}\right)^{\frac{1}{M-2}}\right)$, and $arccos(\cdot)$ is   the inverse of the cosine function. 
We denote the complementary   of $\mathcal{A}$ as $\mathcal{A}^c = \Omega\setminus\mathcal{A}$, i.e., 
\begin{equation*}\label{eq:the_set}
    \resizebox{1.05\linewidth}{!}{$\mathcal{A}^c = \left\{z_1, z_2, \mathbf{h}, \mathbf{g}: z_1, z_2\sim \mathcal{N}(0,1),  \mathbf{h}, \mathbf{g}\sim \mathcal{U}(\mathbb{V}_{1,M}),  \left|\theta-\frac{\pi}{2}\right| \geq  \theta_0\right\}.$}
\end{equation*}
Since $z_1$ and $z_2$ are independent of $\mathbf{h}$ and $\mathbf{g}$, by applying   Lemma \ref{lemma:angle} and setting $P=M$ and $\sqrt{\pi}\frac{\Gamma(\frac{P}{2})}{\Gamma(\frac{P-1}{2})} cos(\theta_0)^{P-2}=\delta$, we have $\Pr[\mathcal{A}^c] \leq  \delta$.


% Since $\mathrm{PLRV}^{(\mathbf{s})}_{(R1SMG(\bm{x})||R1SMG(\bm{x}'))}$ in (\ref{eq:plrv-r1smg}) considers the   log-ratio of the probability densities $\Pr[f(\bm{x})+\mathbf{n} = \mathbf{s}]$ and $\Pr[f(\bm{x}')+\mathbf{n}'= \mathbf{s}]$, it implies that the support (i.e., sampling space) of $\mathrm{PLRV}^{(\mathbf{s})}_{(R1SMG(\bm{x})||R1SMG(\bm{x}'))}$ is $\mathcal{E}\cap \mathcal{E}'$, i.e., 
% \begin{equation*} 
% \begin{aligned}
% \mathcal{E}\cap\mathcal{E}' = &\Big\{z_1, z_2, \mathbf{h}, \mathbf{g}: z_1, z_2\sim \mathcal{N}(0,1),  \mathbf{h}, \mathbf{g}\sim \mathcal{U}(\mathbb{V}_{1,M}), \\
% & f(\bm{x})+\sqrt{\sigma_*}z_1\mathbf{h} = \mathbf{s}\in \mathcal{S}, f(\bm{x}')+\sqrt{\sigma_*}z_2\mathbf{g} = \mathbf{s}\in \mathcal{S}\Big\}.
% \end{aligned}
% \end{equation*}

% By rewirting the support of $\mathrm{PLRV}^{(\mathbf{s})}_{(R1SMG(\bm{x})||R1SMG(\bm{x}'))}$ as 
Since $\mathcal{T} = \big(\mathcal{T} \cap\mathcal{A}\big) \cup   \big(\mathcal{T}\cap \mathcal{A}^c\big)$, we have%\footnote{Note that $\Pr[\mathrm{PLRV}^{(\mathbf{s})}_{(R1SMG(\bm{x})||R1SMG(\bm{x}'))}] = $} 
\begin{equation*}
\begin{aligned}
    \Pr[\mathcal{T}] = &   \Pr[\mathcal{T}\cap\mathcal{A}] + \Pr[\mathcal{T}\cap\mathcal{A}^c] 
    \leq   \Pr[\mathcal{T}\cap\mathcal{A}] + \Pr[\mathcal{A}^c]\\ \leq   &\Pr[\mathcal{T}\cap\mathcal{A}] +  \delta \\
    \leq & 1,
\end{aligned}
\end{equation*}
which suggests $\Pr[\mathcal{T}\cap\mathcal{A}]\leq 1-\delta$. Comparing   with (\ref{eq:plrv-r1smg}), it suffices to show that
\begin{equation}\label{eq:needs-show}
\ln\left(\frac{\Pr[f(\bm{x})+\mathbf{n} = \mathbf{s}]}{\Pr[f(\bm{x}')+\mathbf{n}'= \mathbf{s}]}\right) \leq \epsilon,\quad 
\forall   (z_1,z_2,\mathbf{h},\mathbf{g})\in \mathcal{T}\cap  \mathcal{A}.
\end{equation}



% For neighboring  dataset  $\bm{x}$ and $\bm{x}'$ , we consider the   events  $\mathcal{E}$ and $\mathcal{E}'$, which are respectively defined as follows.
% \begin{equation*} 
% \begin{aligned}
%         &\resizebox{1.07\linewidth}{!}{$\mathcal{E} = \left\{z_1, z_2, \mathbf{h}, \mathbf{g}: z_1, z_2\sim \mathcal{N}(0,1),  \mathbf{h}, \mathbf{g}\sim \mathcal{U}(\mathbb{V}_{1,M}), f(\bm{x})+\sqrt{\sigma_*}z_1\mathbf{h} = \mathbf{s}\in \mathcal{S}\right\},$}\\
%      &\resizebox{1.07\linewidth}{!}{$\mathcal{E}' = \left\{z_1, z_2, \mathbf{h}, \mathbf{g}: z_1, z_2\sim \mathcal{N}(0,1),  \mathbf{h}, \mathbf{g}\sim \mathcal{U}(\mathbb{V}_{1,M}), f(\bm{x}')+\sqrt{\sigma_*}z_2\mathbf{g}= \mathbf{s}\in \mathcal{S}\right\}.$}
% \end{aligned}
% \end{equation*}
% Here, $\mathcal{S}$ is all possible outputs of the proposed R1SMG mechanism. Clearly, $\mathcal{E}$ and $\mathcal{E}'$
% are also  subsets of $\mathcal{T}$.


% Next, we have
% \begin{equation*} 
% \begin{aligned}
% \mathcal{E}\cap\mathcal{A} = \Big\{&z_1, z_2, \mathbf{h}, \mathbf{g}: z_1, z_2\sim \mathcal{N}(0,1),  \mathbf{h}, \mathbf{g}\sim \mathcal{U}(\mathbb{V}_{1,M}), \\
% &\left|\theta-\frac{\pi}{2}\right| \geq  \theta_0, f(\bm{x})+\sqrt{\sigma_*}z_1\mathbf{h}\in \mathcal{S}\Big\}, \quad \text{and}\\
% \mathcal{E}'\cap\mathcal{A} = \Big\{&z_1, z_2, \mathbf{h}, \mathbf{g}: z_1, z_2\sim \mathcal{N}(0,1),  \mathbf{h}, \mathbf{g}\sim \mathcal{U}(\mathbb{V}_{1,M}), \\
% &\left|\theta-\frac{\pi}{2}\right| \geq  \theta_0, f(\bm{x})+\sqrt{\sigma_*}z_2\mathbf{g}\in \mathcal{S}\Big\}.
% \end{aligned}
% \end{equation*}

% Based on Definition \ref{def_dp}, R$1$SMG achieves $(\epsilon,\delta)$-DP   for all possible output $\mathcal{S}$ if  %it satisfies that
% \begin{gather}
% % \resizebox{0.9\hsize}{!}{$
% \Pr[f(\bm{x})+\mathbf{n} \in  \Ss]\leq e^{\epsilon} \Pr[f(\bm{x}')+\mathbf{n}' \in  \Ss ]+\delta.
% %$}
% \label{AMGIC_dp}
% \end{gather}
% Then, for the left hand-side of (\ref{AMGIC_dp}), we can have 
% \begin{equation*}
% \begin{aligned}
% &\Pr [f(\bm{x})+\mathbf{n}\in\Ss ]\\
% =&\Pr [   (\{      f(\bm{x}) +\mathbf{n}     \in\Ss\}  \cap \mathcal{A})  \cup   (\{     f(\bm{x}) +\mathbf{n}\in\Ss\}  \cap \mathcal{A}^c)   ] \\
% = & \Pr   [\{      f(\bm{x}) +\mathbf{n}     \in\Ss\}  \cap \mathcal{A} ]+\Pr    [\{      f(\bm{x}) +\mathbf{n}     \in\Ss\}  \cap \mathcal{A}^c ]\\
% \leq & \Pr   [\{     f(\bm{x}) +\mathbf{n}     \in\Ss\}  \cap \mathcal{A}] + \Pr [ \mathcal{A}^c]\\
% \leq & \Pr   [  f(\bm{x}) +\mathbf{n}     \in(\Ss  \cap \mathcal{A})] + \delta.
% \end{aligned}
% \end{equation*}
% For the right hand-side of (\ref{AMGIC_dp}), we can directly have
% \begin{gather*}
% \begin{aligned}
%     e^{\epsilon} \Pr [ f(\bm{x}')+\mathbf{n}'\in  \Ss ]+\delta\geq e^{\epsilon} \Pr [f(\bm{x}')+\mathbf{n}'\in  (\Ss\cap\mathcal{A}) ] + \delta.
%    \end{aligned}
% \end{gather*}
Since $\mathbf{n}$ (resp. $\mathbf{n}'$) is singular multivariate Gaussian with zero mean by design (see (\ref{mapping2})). 
Thus $f(\bm{x})+\mathbf{n} = \mathbf{s}\in \mathcal{S}$  (resp. $f(\bm{x}')+\mathbf{n}' = \mathbf{s}\in \mathcal{S}$) is attributed to singular multivariate  Gaussian distribution, with mean $f(\bm{x})$ (resp. $f(\bm{x}')$) and covariance matrix $\mathbf{h} \sigma_* \mathbf{h}^T$ (resp. $\mathbf{g} \sigma_*  \mathbf{g}^T$) (one can verify this by setting $r=1$ in (\ref{eq:emp-covariance})). Plugging the mean and generalized inverse covariance matrix into the PDF provided in Definition \ref{def:singular_pdf} (with $r=1$), we have 
\begin{equation*}
\begin{aligned}
&\mathrm{PLRV}^{(\mathbf{s})}_{(R1SMG(\bm{x})||R1SMG(\bm{x}'))} = \ln\left(\frac{\Pr[f(\bm{x})+\mathbf{n} = \mathbf{s}]}{\Pr[f(\bm{x}')+\mathbf{n}'= \mathbf{s}]}\right)\\
=& \resizebox{0.98\linewidth}{!}{$\ln\left(\frac{{(2\pi)^{-\frac{1}{2}}    \exp\left(-\frac{1}{2}  \big(\mathbf{s}-f(\bm{x})\big)^T \big(\mathbf{h} \sigma_*^{-1} \mathbf{h}^T\big) \big(\mathbf{s}-f(\bm{x})\big)\right)       }\Big/{\sqrt{\sigma_*}}}{{(2\pi)^{-\frac{1}{2}}    \exp\left(-\frac{1}{2}  \big(\mathbf{s}-f(\bm{x}')\big)^T \big(\mathbf{g} \sigma_*^{-1} \mathbf{g}^T\big) \big(\mathbf{s}-f(\bm{x}')\big)\right)       }\big/{\sqrt{\sigma_*}}}\right)$}\\
= &  \ln\left( \frac{\exp\left (-\frac{1}{2\sigma_*}    \Big(  \mathbf{h}^T(\mathbf{s}-f(\bm{x}))   \Big)^2    \right )}{\exp\left (-\frac{1}{2\sigma_*}    \Big( \mathbf{g}^T(\mathbf{s}-f(\bm{x}'))   \Big)^2\right )} \right) \\
=&\frac{1}{2\sigma_*}  \left(    \Bigg(  \underbrace{ \mathbf{g}^T (\mathbf{s}-f(\bm{x}')) }_{\rho_1\in \R}  \Bigg)^2  - \Bigg( \underbrace{ \mathbf{h}^T (\mathbf{s}-f(\bm{x})) }_{\rho_2\in \R}\Bigg)^2  \right)\\
\leq & \frac{1}{2\sigma_*}  \Big(|\rho_1|+|\rho_2|\Big)^2.
\end{aligned}
\end{equation*}
% \begin{equation}\label{eq:diverge_begin}
% \begin{aligned}
% &\mathrm{PLRV}_{\mathcal{M}_{R1SMG},\bm{x},\bm{x}'} = \left|\ln\left( \frac{\exp{\Big\{-\frac{1}{2}    \Big( \sigma_*^{-1/2}\mathbf{h}^T(\mathbf{s}-f(\bm{x}))   \Big)^2}\Big\}}{\exp{\Big\{-\frac{1}{2}    \Big( \sigma_*^{-1/2}\mathbf{g}^T(\mathbf{s}-f(\bm{x}'))   \Big)^2}\Big\}} \right)\right|\leq  \epsilon\\
% \Leftrightarrow & \frac{1}{2\sigma_*}\times \left|    \Bigg(  \underbrace{ \mathbf{g}^T (\mathbf{s}-f(\bm{x}')) }_{\rho_1\in \R}  \Bigg)^2  - \Bigg( \underbrace{ \mathbf{h}^T (\mathbf{s}-f(\bm{x})) }_{\rho_2\in \R}\Bigg)^2  \right| \leq \epsilon.
% \end{aligned}
% \end{equation}
% Factorizing the difference of squares gives %, for the left hand side of  (\ref{eq:diverge_begin}), we    have 
% \begin{equation}\label{eq:our_goal}
% \begin{aligned}
%        & \frac{1}{2\sigma_*} |(\rho_1-\rho_2)  (\rho_1+\rho_2)|\\ \leq & \frac{1}{2\sigma_*}   |\rho_1-\rho_2|  |\rho_1+\rho_2| \leq  \frac{1}{2\sigma_*}  (|\rho_1|+|\rho_2|)^2.
% \end{aligned}
% \end{equation}
 In what follows, we derive  tight upper bound on   $|\rho_1|+|\rho_2|$. 
In particular, with $||\mathbf{g}||_2 = ||\mathbf{h}||_2=1$, we    notice that
\begin{gather*}
\begin{aligned}
 |\rho_1|+|\rho_2| 
 & \leq ||\mathbf{g}||_2||\mathbf{s}-f(\bm{x}')||_2 + ||\mathbf{h}||_2||\mathbf{s}-f(\bm{x})||_2\\
 &  =  ||\mathbf{s}-f(\bm{x}')||_2 +  ||\mathbf{s}-f(\bm{x})||_2,
\end{aligned}
\end{gather*}
Thus, we just need to   bound   $||\mathbf{s}-f(\bm{x}')||_2 +  ||\mathbf{s}-f(\bm{x})||_2$. 


 






First, we observe that the angle between $(\mathbf{s}-f(\bm{x}))$ and  $(\mathbf{s}-f(\bm{x}'))$ is      identical to the angle between $\mathbf{h}$ and $\mathbf{g}$, because    $(\mathbf{s}-f(\bm{x}))=\mathbf{n}$ and $(\mathbf{s}-f(\bm{x}'))=\mathbf{n}'$, and $\mathbf{n}$ and $\mathbf{n}'$ are obtained by   scaling $\mathbf{h}$ and $\mathbf{g}$. % (i.e., $\mathbf{n}\in Span(\mathbf{h})$ and $\mathbf{n}'\in Span(\mathbf{h})$). 
We use $\theta$ to represent the angle between $\mathbf{h}$ and $\mathbf{g}$ (i.e.,  identically between $(\mathbf{s}-f(\bm{x}))$ and $(\mathbf{s}-f(\bm{x}'))$). Thus, from a geometric perspective, $||\mathbf{s}-f(\bm{x}')||_2 +  ||\mathbf{s}-f(\bm{x})||_2$ is the sum of the length of two edges of a triangle in $\R^{M}$, and the angle between these two edges is $\theta$. Moreover, the length of the third edge (opposite to this specific angle) is $|| (\mathbf{s}-f(\bm{x}')) - (\mathbf{s}-f(\bm{x}))||_2 
  =||f(\bm{x})- f(\bm{x}') ||_2$.
% $||\mathbf{n}' - \mathbf{n}||_2=|| (\mathbf{s}-\bm{x}') - (\mathbf{s}-f(\bm{x}))||_2 
%   =||\text{vec}(f(\bm{x}')^T)-\text{vec}(f(\bm{x}')^T) ||_2$.
% % \begin{equation}
% % \begin{aligned}
% %     \Big|\Big|\mathbf{n}' - \mathbf{n} \Big|\Big|_2&=\Big|\Big| (\mathbf{s}-\bm{x}') - (\mathbf{s}-f(\bm{x}))\Big|\Big|_2\\
% %   &=\Big|\Big|\text{vec}(f(\bm{x}')^T)-\text{vec}(f(\bm{x}')^T) \Big|\Big|_2. %\leq \Delta_2f,  
% %     \end{aligned}
% % \end{equation}
% Thus, from a geometric perspective, $||(\mathbf{s}-\bm{x}')||_2 +  ||(\mathbf{s}-f(\bm{x}))||_2$ is the sum of the length of two edges of a triangle in $\R^{MN\times 1}$. The third edge of this specific triangle has length $||\text{vec}(f(\bm{x}')^T)-\text{vec}(f(\bm{x}')^T) ||_2$. The angle opposite to the third edge  is identical to the angle between $\mathbf{h}$ and $\mathbf{g}$, because    $\mathbf{n}$ and $\mathbf{n}'$ are obtained by   scaling $\mathbf{h}$ and $\mathbf{g}$ (i.e., $\mathbf{n}\in Span(\mathbf{h})$ and $\mathbf{n}'\in Span(\mathbf{h})$). We use $\theta$ to represent the angle between $\mathbf{h}$ and $\mathbf{g}$ (i.e.,  identically between $(\mathbf{s}-f(\bm{x}))$ and $(\mathbf{s}-\bm{x}')$). 
% % Clearly, 
For better understanding, we visualize the above description   in Figure \ref{fig:geometric}(a), where the red point (resp. blue point) indicates $\mathbf{n}$ (resp. $\mathbf{n}'$) in $\R^{M}$, and the red dashed line (resp. blue dashed line) is the randomly sampled $\mathbf{h}$ (resp. $\mathbf{g}$) (note that we show $\mathbf{h}$ and $\mathbf{g}$ as bidirectional, because $\mathbf{n}$ and $\mathbf{n}'$ can point to the opposite direction of $\mathbf{h}$ and $\mathbf{g}$, respectively).

\begin{figure}[htb]
  \begin{center}
     \includegraphics[width= 0.8\columnwidth]{figure_noise_sample_compare/crypto23_r1smg.jpg}\\
       \end{center}
  \caption{\label{fig:geometric}(a) Geometric interpretation of $|\rho_1|+|\rho_2|$.   Circumcircles of the described triangle with (b) $\theta<\frac{\pi}{2}$ and (c) $\theta>\frac{\pi}{2}$.}
\end{figure}


It is well know that the length of each edge of a triangle is upper bounded by  the diameter  of the circumscribed circle of the triangle. We demonstrate this fact in Figure \ref{fig:geometric}(b) and (c), where $\frac{d}{2}$ represents the  radius of the circumcircle.  According to the law of sine, we have $d =   ||f(\bm{x})-f(\bm{x}')  ||_2\big/{sin(\theta)}$. Thus, 
\begin{equation}\label{eq:plrv_r1smg}
\begin{aligned}
&||\mathbf{s}-f(\bm{x}')||_2 +  ||\mathbf{s}-f(\bm{x})||_2 
\\
\leq & 2d = 2||f(\bm{x})-f(\bm{x}')||_2\big/{sin(\theta)}\leq \frac{2\Delta_2 f}{sin(\theta)},
\end{aligned}
\end{equation}
where the last inequality is because the query sensitivity on neighboring datasets is $\Delta_2f = \max_{\bm{x},\bm{x}'}||f(\bm{x})-f(\bm{x}')||_2$. % (i.e., Definition \ref{sens_def}).

Since we consider $(z_1,z_2,\mathbf{h},\mathbf{g})\in \mathcal{T}\cap  \mathcal{A}$, we have $\theta\in(\frac{\pi}{2}-\theta_0,\frac{\pi}{2}+\theta_0)$, $\theta_0\in[0,\frac{\pi}{2}]$, and due to the symmetry of sine function around $\frac{\pi}{2}$, the maximum value of $\frac{2\Delta_2f}{sin(\theta)}$ is smaller than   $\frac{2\Delta_2f}{sin(\frac{\pi}{2}-\theta_0)}$, which is equivalent to $\frac{2\Delta_2f}{cos(\theta_0)}$. Since 
  $\theta_0 = arccos\left(\left(\frac{\delta\Gamma(\frac{M-1}{2})}{\sqrt{\pi}\Gamma(\frac{M}{2})}\right)^{\frac{1}{M-2}}\right)$ (given in event $\mathcal{A}$), we have
  \begin{small}
      \begin{gather*}
\begin{aligned}
|\rho_1| +|\rho_2| \leq  &  ||\mathbf{s}-f(\bm{x}')||_2 + ||\mathbf{s}-f(\bm{x})||_2 \\
  <&  %\frac{2\Delta_2f}{sin(\frac{\pi}{2}-\theta_0)} =
  \frac{2\Delta_2f}{cos(\theta_0)} = 2\Delta_2f\Bigg/\left(\frac{\delta\Gamma(\frac{M-1}{2})}{\sqrt{\pi}\Gamma(\frac{M}{2})}\right)^{\frac{1}{M-2}}. % = \frac{2\Delta_2f}{\sqrt{\psi}}.
\end{aligned}
\end{gather*}
  \end{small}





Combining the above results with (\ref{eq:needs-show}), we obtain the sufficient condition for the proposed R$1$SMG to achieve $(\epsilon,\delta)$-differential privacy as $\frac{1}{2\sigma_*} ( |\rho_1|+|\rho_2| )^2  \leq \frac{1}{2\sigma_*}  \left(2\Delta_2f\Bigg/\left(\frac{\delta\Gamma(\frac{M-1}{2})}{\sqrt{\pi}\Gamma(\frac{M}{2})}\right)^{\frac{1}{M-2}}\right)^2\leq \epsilon 
  \Leftrightarrow  
  \sigma_*\geq \frac{2\Delta_2f^2}{\epsilon\psi}$.
% \begin{equation*}
% \begin{aligned}
% &  \frac{1}{2\sigma_*} ( |\rho_1|+|\rho_2| )^2  \leq \frac{1}{2\sigma_*}  \left(2\Delta_2f\Bigg/\left(\frac{\delta\Gamma(\frac{M-1}{2})}{\sqrt{\pi}\Gamma(\frac{M}{2})}\right)^{\frac{1}{M-2}}\right)^2\leq \epsilon\\
%   \Leftrightarrow &
%   \sigma_*\geq \frac{2\Delta_2f^2}{\epsilon\psi}, 
% \end{aligned}
% \end{equation*}
% i.e., $\sigma_*^{-1/2}\sqrt{\omega}\Bigg(\frac{\Delta_2f}{\sqrt{\psi}}\Bigg)\leq \epsilon$, 
% % \begin{equation*}
% %     \sigma_*^{-1/2}\frac{2\Delta_2f\sqrt{\omega}}{sin(\frac{\pi}{2}-\theta_0)}\leq 2\epsilon,
% % \end{equation*}
% which is equivalent to 
% \begin{gather*}
%     \sigma_*\geq \frac{\Delta_2f^2\omega}{\epsilon^2\psi} = {\Delta_2f^22\Big( 2\sqrt{- \ln\delta_1}-2\ln\delta_1+1\Big)}\Bigg/\left(\epsilon^2 \left(\frac{(1-\delta_2)\Gamma(\frac{MN-1}{2})}{\sqrt{\pi}\Gamma(\frac{MN}{2})}\right)^{\frac{2}{MN-2}}\right)
% \end{gather*}
% the conclusion of Theorem \ref{thm_multivariate} and 
\end{proof}




%\vspace{-8mm}
\textbf{Practical Implementation of R1SMG.} 
%The remaining question on the application  of   R$1$SMG is   sampling variable from $\mathbb{V}_{1,M}$. 
According to Theorem \ref{thm:sample_V}, we can obtain the desired random variable supported on the Stiefel manifold by transforming samples drawn i.i.d. from standard Gaussian distribution.  As a result, we can apply Theorem \ref{thm:sample_V} with $r=1$ to draw the desired samples  from $\mathbb{V}_{1,M}$.
\begin{theorem}[Generating Random Samples from $\mathbb{V}_{r,M}$ (see page 29, Theorem 2.2.1.(iii) of \cite{chikuse2012statistics})]\label{thm:sample_V}Let $\mathbf{x}\in\R^{M\times r}$, whose elements are i.i.d. sampled from $\mathcal{N}(0,1)$. Then $\mathbf{v} = \mathbf{x}(\mathbf{x}^T\mathbf{x})^{-1/2}$ is uniformly distributed on $\mathbb{V}_{r,M}$.
\end{theorem}




% \subsubsection{Curse Lifted.}\label{sec:curse_lifited} 


\subsection{Asymptotic Behavior}\label{sec:discussion_r1smg}

\textbf{Curse Lifted.} 
At this point, we can do a quick sanity check that the expected accuracy loss introduced by R$1$SMG is $\Tr[\bm{\Pi}]$, which  is not the summation of $M$ positive values any more.  Specifically, 
\begin{gather}
\begin{aligned}
       &\mathbb{E}_{R1\mathrm{SMGM}}[\L] =  \mathbb{E}[||\mathbf{n}||_2^2] \\
       =&\mathbb{E}_{\mathclap{\substack{\\\\\\  z\sim \mathcal{N}(0,1),\mathbf{v}\sim\mathcal{U}(\mathbb{V}_{1,M})}}}\Big[ (\mathbf{v}   \sigma_*^{1/2}z)^T\mathbf{v}   \sigma_*^{1/2}z ] = \sigma_*\mathbb{E}[z^2] = \sigma_* 
\end{aligned}
    \label{eq:freedom_r}
\end{gather}
and the last equality holds because $z^2\sim\chi^2(1)$ and the expected value of chi-squared distributed variable is its degree of freedom.
% where $(a)$ follows from  $\mathbf{V}_r^T\mathbf{V}_r = \mathbf{I}_{r\times r}$, and $(b)$ is obtained by noticing that $\mathbf{z}^T\bm{\Lambda}_r\mathbf{z}$ is a quadratic form of $\mathbf{z}\sim\mathcal{N}(\mathbf{0},\mathbf{I}_{r\times r})$ with $\A = \bm{\Lambda}_r$, and then applying  Theorem \ref{m}
%  with $t=1$. 
(\ref{eq:freedom_r}) clearly shows that we have lifted the identified curse by considering noises attributed to a singular multivariate Gaussian distribution with rank 1 covariance matrix.  


Moreover, we prove that $\mathbb{E}_{R1\mathrm{SMGM}}[\L]$ decreases with dimension of the query result ($M$), and if $M$ goes to infinity, $\mathbb{E}_{R1\mathrm{SMGM}}[\L]$ converges to a constant, which means only constant amount of noise is need to perturb $f(\bm{x})\in\R^M$. %Property \ref{claim:magic_claim} is formalized in the next Theorem.
\begin{theorem}\label{theorem:r1smg_asymptotic} For any fixed $\epsilon>0,0<\delta<1$, $\mathbb{E}_{R1\mathrm{SMGM}}[\L]$ monotonically decreases with $M$. 
When $M\rightarrow +\infty$, $\mathbb{E}_{R1\mathrm{SMGM}}[\L] \rightarrow \frac{2(\Delta_2f)^2}{\epsilon}$.
\end{theorem}
\begin{proof} First we have
\begin{equation*}
\begin{aligned}
&\frac{2\Delta_2f^2}{\epsilon \psi}  = \frac{2\Delta_2f^2}{\epsilon} \left(\frac{\sqrt{\pi}\Gamma(\frac{M}{2})}{\delta\Gamma(\frac{M-1}{2})}\right)^{\frac{2}{M-2}} \\=& \frac{2\Delta_2f^2}{\epsilon} \exp\left(  \frac{2}{M-2} \ln\left(\frac{\sqrt{\pi}\Gamma(\frac{M}{2})}{\delta\Gamma(\frac{M-1}{2})}\right)\right).  
\end{aligned}
\end{equation*}
Then, to analyze $\frac{\Gamma(\frac{M}{2})}{\Gamma(\frac{M-1}{2})}$, we observe that its reciprocal is related to 
the normalization constant of the PDF of the Beta distribution $Beta(\alpha,\beta)$. In particular, the normalization constant $B(\alpha,\beta)$ of $Beta(\alpha,\beta)$ is defined in terms of Gamma function, i.e., $B(\alpha,\beta) = \frac{\Gamma(\alpha)\Gamma(\beta)}{\Gamma(\alpha+\beta)}$. Thus  $B(\frac{M-1}{2},\frac{1}{2}) = \frac{\Gamma(\frac{M-1}{2})\Gamma(\frac{1}{2})}{\Gamma(\frac{M}{2})} = \sqrt{\pi}\frac{\Gamma(\frac{M-1}{2})}{\Gamma(\frac{M}{2})}$. It suggests  that 
\begin{equation*}
\begin{aligned}
        &\frac{\Gamma(\frac{M-1}{2})}{\Gamma(\frac{M}{2})} = \frac{1}{\sqrt{\pi}}B\left(\frac{M-1}{2},\frac{1}{2}\right) \stackrel{(*)}= \frac{1}{\sqrt{\pi}} \int_0^1 x^{\frac{M-3}{2}} (1-x)^{-\frac{1}{2}} dx \\
        =& \frac{2}{\sqrt{\pi}}\int_0^1 \frac{x^{M-2}}{\sqrt{1-x^2}}dx = \frac{2}{\sqrt{\pi}}\int_0^{\frac{\pi}{2}} cos^{M-2} \eta d \eta \\
        =& \frac{2}{\sqrt{\pi}}\int_0^\infty \exp\left(-(M-2) \frac{\eta^2}{2}\right) d\eta = \frac{\sqrt{2}}{\sqrt{M-2}},
\end{aligned}
\end{equation*}
where $(*)$ is obtained by plugging the PDF of $Beta(\frac{M-1}{2},\frac{1}{2})$. As a result, $\frac{\Gamma(\frac{M}{2})}{\Gamma(\frac{M-1}{2})} = \frac{\sqrt{M-2}}{\sqrt{2}}$, hence, $\frac{2\Delta_2f^2}{\epsilon \psi}  = \frac{2\Delta_2f^2}{\epsilon}\exp\left(   \frac{2}{M-2} \ln\left(\frac{\sqrt{\pi}}{\delta} \frac{\sqrt{M-2}}{\sqrt{2}}\right)\right)$, which is a monotonically decreasing function w.r.t. $M$.

When $M\rightarrow \infty$, we have  
\begin{equation*}
    \begin{aligned}
        \lim_{M\rightarrow \infty}  \frac{2\Delta_2f^2}{\epsilon \psi} = &  \frac{2\Delta_2f^2}{\epsilon} \exp\left(\lim_{M\rightarrow \infty}  \frac{2}{M-2} \ln\left(\frac{\sqrt{\pi}}{\delta} \frac{\sqrt{M-2}}{\sqrt{2}}\right)\right)\\
      \stackrel{(*)}   = &      \frac{2\Delta_2f^2}{\epsilon}  \exp(0) =    \frac{2\Delta_2f^2}{\epsilon},
    \end{aligned}
\end{equation*}
where   $(*)$ is due to the l'H\^{o}pital's Rule. %The proof is completed. 
% \begin{equation*}
% \begin{aligned}
%     \lim_{M\rightarrow \infty}  \frac{2\Delta_2f^2}{\epsilon \psi} & = \lim_{M\rightarrow \infty}  \frac{2\Delta_2f^2}{\epsilon} \left(\frac{\sqrt{\pi}\Gamma(\frac{M}{2})}{\delta\Gamma(\frac{M-1}{2})}\right)^{\frac{2}{M-2}}\\
%     & = \frac{2\Delta_2f^2}{\epsilon} \exp\left(\lim_{M\rightarrow \infty}  \frac{2}{M-2} \ln\left(\frac{\sqrt{\pi}\Gamma(\frac{M}{2})}{\delta\Gamma(\frac{M-1}{2})}\right)\right).
% \end{aligned}
% \end{equation*}
\end{proof}
\begin{remark}\label{remark:converge_pi2}
The ``magic'' (the expected accuracy loss decreases with $M$) can also be interpreted from a geometric perspective. From the proof of Theorem \ref{thm_multivariate}, we know $\sigma_* = \frac{2(\Delta_2f)^2}{\epsilon sin^2(\theta)}$, where   $\theta$ is the angle between the noises ($\mathbf{n}$ and $\mathbf{n}'$) used to perturb $f(\bm{x})$ and $f(\bm{x}')$. Since $\mathbf{n}$ and $\mathbf{n}'$ are scaled variables sampled from the unit sphere, and as the dimension increases, the angle $\theta$  quickly concentrates around $\frac{\pi}{2}$ (at the rate of $\sqrt{M}$ \cite{cai2013distributions}).
\end{remark}


In Appendix \ref{sec:explain-property}, we provide an intuitive explanation of the unique property of R1SMG by using a set of $M$ counting queries as an example. In Appendix \ref{sec:versus_M}, we plot the empirical $\mathbb{E}[\L]$ versus $M$ achieved by R1SMG and other mechanisms, and clearly show that $\mathbb{E}_{R1SMG}[\L]$ monotonically decrease with $M$, whereas the other increase with $M$ (cf. Figure \ref{fig:scale_study}).

% experimentally show

% \input{sections/waste-of-gaussian}



\subsection{Discussion on Privacy Leakage of Utilizing Sensing Vector in the Null Space of $\mathbf{v}$}\label{sec:null_space_attack}

Our proposed R$1$SMG does not span the entire space of $\R^{M}$, thus, it may raise  concern of privacy leakage if one can take advantage of  the  sensing      vector  in the null space of $\mathbf{v}$. To be more specific, let $\mathbf{s}$ be the output of R$1$SMG and $\mathbf{u}\in Null(\mathbf{v})$, i.e., $<\mathbf{u},\mathbf{v}>=0$. Since $\mathbf{n}\in Span(\mathbf{v})$, one can have
\begin{equation*}
    <\mathbf{u},\mathbf{s}> = <\mathbf{u},f(\bm{x})+\mathbf{n}> = <\mathbf{u},f(\bm{x})>,
\end{equation*}
implying potential privacy leakage of   linear queries on $f(\bm{x})$.

However, we need to highlight that $\mathbf{v}$ is randomly sampled from $\mathcal{U}(\mathbb{V}_{1,M})$, which is an intermediate noise to produce the final noise of  R$1$SMG  and will not be made public (the other intermediate noise is $z$). Note that this is not  against the core idea of differential privacy, i.e., ``privacy without obscurity", because the entire noise generation process, i.e, (\ref{mapping2}), including  the choice of  distribution parameters are transparent.  As a result, the probability that a constructed $\mathbf{u}$ that is in the null space of a randomly sampled $\mathbf{v}$ is zero, i.e., %$\Pr[\mathbf{u}\in Span(\mathbf{v})] = 0$. The reason is that  
$\Pr[\mathbf{u}\in Null(\mathbf{v})] = \frac{\mu(Null(\mathbf{v}))}{\mu(\mathbb{R}^{M})} = 0$, where $\mu(\cdot)$ denotes the Lebesgue measure of a measurable set.
%\vspace{-4mm}
\begin{figure}[htb]
  \begin{center}
     \includegraphics[width= 0.8 \columnwidth]{figure_noise_sample_compare/manifold_toy (2).png}
       \end{center}%\vspace{-4mm}
  \caption{\label{fig:manifold_toy}Visualization of the null space of the noise generated by R$1$SMG. Left: $\mathbb{V}_{1,2}$. Right: $\mathbb{V}_{1,3}$.}
\end{figure}
%\vspace{-4mm}

For better explanation, we give   toy examples in $\R^2$ and $\R^3$ (when $M=2$ and $M=3$). Particularly, in $\R^2$, $\mathbb{V}_{1,2}$ is the unit circle shown in Figure \ref{fig:manifold_toy} (left). Suppose $\mathbf{v}_1 = [-1/\sqrt{5},2/\sqrt{5}]^T$ is the randomly sampled variable in $\mathbb{V}_{1,2}$, then $Null(\mathbf{v}_1)$ is   $\mathcal{I}$ (the dashed line orthogonal to $\mathbf{v}_1$). Clearly, the probability of sampling a point from $\R^2$ that resides on a specific line is 0. Likewise, in $\R^3$, $\mathbb{V}_{1,3}$ is the unit sphere shown in Figure \ref{fig:manifold_toy} (right). Suppose $\mathbf{v}_2 = [1/\sqrt{3},-1/\sqrt{3},1/\sqrt{3}]^T$ is the randomly sampled variable in $\mathbb{V}_{1,3}$, then $Null(\mathbf{v}_2)$ is    $\mathcal{F}$ (the   plane orthogonal to $\mathbf{v}_2$). The probability of sampling a point from $\R^3$ that resides on a specific plane is also 0. Although, it is publicly known that $\mathbf{v}$ is   sampled from $\mathcal{U}(\mathbb{V}_{1,M})$, the Lebesgue measure of $Null(\mathbf{v})$ (given $\mathbf{v}\subset\mathbb{V}_{1,M}$) is still 0. For example, the probability of sampling the blue points in Figure \ref{fig:manifold_toy} (left) is 0, and the probability of sampling points residing on $\mathcal{C}\subset\mathcal{F}$ (the circle orthogonal to $\mathbf{v}_2$) in Figure \ref{fig:manifold_toy} (right) is also 0. 
Hence, by generating $\mathbf{v}$ randomly, the proposed R$1$SMG will cause privacy leakage under linear query with probability zero. 







% \subsubsection{Determining $\delta_1$ and $\delta_2$ in R$1$SMG}\label{sec:assign_delta} %First, we need  to determine the value of $\delta_1$ and $\delta_2$ given the budget of $\delta$. 
% Noe that for any $(\epsilon,\delta)$-differential privacy requirement, as long as the determined $\delta_1$ and $\delta_2$ satisfy $\delta_1+\delta_2-\delta_1\delta_2 = \delta$, we can achieve the same differential privacy guarantee. From (\ref{eq:freedom_r}) we know that given the budget of $\delta$, different allocation of $\delta_1$ and $\delta_2$  may lead to different expected accuracy loss. Thus, one can solve for the optimal $\delta_1$ and $\delta_2$ by minimizing $\mathbb{E}_{1\mathrm{SMGM}}[\L]$ under the constraint of a provided value of $\delta$. However, this formulated problem will be non-convex and difficult to solve. Actually, by   equally allocating the budget of $\delta$ to $\delta_1$ and $\delta_2$,  we can already achieve lower expected accuracy loss than other variants of Gaussian mechanisms. In the following sections, we will show that if $\delta_1 = \delta_2$, R$1$SMG can boost the utility of query results (see Theorem \ref{utility_compare} and Corollary \ref{thm:g_mvg_accuracy}) and achieve higher utility stability than the variants of Gaussian mechanisms (see Theorem \ref{kk} and \ref{ss}).



% Recall that $\delta_1$ and $\delta_2$ are the probabilities that a squared standard Gaussian random variable exceeding a certain value, and the absolute difference between an random angle and $\frac{\pi}{2}$ is larger than a specific   angle, respectively.  In this work, we only consider   the simplest case where  these two probabilities are equal. 

% In the rest of the paper, we will focus on the analysis (graphically, theoretically, and experimentally) of R$1$SMG  by setting $\delta_1 = \delta_2$. 
% Thus, by solving $\delta = \delta_1+\delta_2-\delta_1\delta_2$ and $\delta_1 = \delta_2$, we obtain $\delta_1 = \delta_2 = 1-\sqrt{1-\delta}$, and immediately have the following corollary. 
% % \begin{corollary}
% R$1$SMG achieves $(\epsilon,\delta)$-differential privacy, if $\sigma_{*} \geq  \frac{\Delta_2f^2 \widetilde{\omega}}{\epsilon^2 \widetilde{\psi}}$, 
% where $\widetilde{\omega}$ and $\widetilde{\psi}$ are given by
% %\vspace{-4mm}
% \begin{gather*}
%     % \begin{aligned}
% %   &
%    \widetilde{\omega} = 2\left( 2\sqrt{- \ln\left(1-\sqrt{1-\delta}\right)}-2\ln\left(1-\sqrt{1-\delta}\right)+1\right),\quad
%    \widetilde{\psi} =  \left(\frac{\left(1-\sqrt{1-\delta}\right)\Gamma(\frac{MN-1}{2})}{\sqrt{\pi}\Gamma(\frac{MN}{2})}\right)^{\frac{2}{MN-2}}.
%     % \end{aligned}
% \end{gather*}
% % $\sigma_{r}$ is the $r$-th largest diagonal value  (i.e., the smallest nonzero diagonal value)  of $\bm{\Lambda}_r$, and $\omega(\delta,r) = 2\sqrt{-r\ln \delta}-2\ln \delta+r$.
% \label{corollary_thm_multivariate}
% % \end{corollary}

% In the rest of the paper, we will focus on the analysis of R$1$SMG (both theoretically and experimentally) by setting  $\delta_1 = \delta_2 = 1-\sqrt{1-\delta}$. The allocation of $\delta_1$ and $\delta_2$ given $\delta$ has impact on the utility of R$1$SMG, and we will  investigate such impact in the future work. For example, please refer to   Section \ref{sec:discussion} for the discussion of a potential solution to achieve higher utility via solving an optimization problem. 






% The time and space complexity of Algorithm \ref{algo:1smgm} are   dominated by the matrix multiplications, which have time   complexity $\mathcal{O}(MN)$ and space complexity $\mathcal{O}(MN)$, because $r=1$. In contrast, the time and space complexity for the MVG mechanism are $\mathcal{O}(M^3N^3)$ and $\mathcal{O}(M^2N^2)$, respectively, because MVG  multiplies 3 matrices of size $MN\times MN$ to generate the noise samples (see Lemma 4 of \cite{Chanyaswad2018}).

% talk about design space...


% \subsubsection{Visualization}


% This is because, given the fixed privacy budget, $\sigma_*$ is proportional to the inverse of an exponential decay function applied on 
% the ratio between two gamma functions of   $MN$. By applying the Stirling's formula \cite{abramowitz1988handbook}, we know that the the ratio between the considered gamma functions scales with $\mathcal{O}(\sqrt{MN})$. Thus, $\sigma_*$ is approximately proportional to $\mathcal{O}(MN^{-1/MN})$, which 
% it explains the nearly stable expected utility loss achieved by 1SMGM (red lines) under varying query size (i.e., $MN$) in Figure \ref{fig:scale_study}.








% We   notice that $\L =||\mathbf{n}||_2^2= \mathbf{n}^T\mathbf{n}$ is a quadratic form in random variable, which is defined as follows.
% \begin{mydef}[Quadratic Form in Random Variable \cite{provost1992quadratic}]
% Denote by $\x$ a random vector with mean $\mathbf{\mu}$ and covariance matrix $\bm{\Xi}$. The quadratic form in random variable $\x$ associated with a symmetric matrix $\A$ is defined as 
% \begin{equation*}
%     Q(\x) = \x^T\A\x.
% \end{equation*}
% \label{quad_def}
% \end{mydef}

% Due to the randomness involved in the perturbation Gaussian noise, $\L$ is nondeterministic. Thus, we investigate    expected value of accuracy loss introduced by the noises, i.e., $\mathbb{E}[\L]$. In the following theorem, we recall the $t$-th moment of quadratic form in Gaussian random variable. 

% \begin{theorem}[\cite{provost1992quadratic}]The $t$-th moment of a quadratic form in multivariate Gaussian random variable, i.e, $\x\sim\mathcal{N}(\mathbf{\mu},\bm{\Xi})$ and $\bm{\Xi}$ is full rank, is given by %$\mathbb{E}[Q(\x)^t] =  \{\sum_{t_1=0}^{t-1}{t-1\choose t_1}g^{(t-1-t_1)}\times \sum_{t_2=0}^{t_1-1}{t_1-1\choose t_2}g^{(t_1-1-t_2)}\times\cdots\times\sum_{t_2=0}^{1}{1-1\choose t_2}g^{(0)} \}$,  
% \begin{equation*}
% \begin{aligned}
% &\mathbb{E}[Q(\x)^t] = \bigg\{\sum_{t_1=0}^{t-1}{t-1\choose t_1}g^{(t-1-t_1)}\times\\
% &\sum_{t_2=0}^{t_1-1}{t_1-1\choose t_2}g^{(t_1-1-t_2)}\times\cdots\times\sum_{t_2=0}^{1}{1-1\choose t_2}g^{(0)}\bigg\},
% \end{aligned}
% \end{equation*}
% where $g^{(k)} = 2^kk!\{\Tr(A\bm{\Xi})^{k+1}+(k+1)\mathbf{\mu}^T(A\bm{\Xi})^kA\mathbf{\mu}\}$,   $k\in[0,t-1]$.
% \label{m}
% \end{theorem}

% We quantify the degradation of utility 

% \section{MGM: An Intermediate Step}
% \label{mgm}





% In this section, we     present the intermediate mechanism, i.e., MGM, and analyze its privacy guarantee. %We start with describing some advantages of the proposed MGM. 



% \begin{mydef}[Multivariate Gaussian Mechanism]
% Given a matrix-valued query $f(D) \in \R^{M\times N}$, MGM is defined as%$\mathcal{MVG}(f(D))  = f(D)+\mathcal{Z}$,
% \begin{equation*}
% \mathbb{MGM}(f(D))  = f(D)+ ({\rm{resize}}(\mathbf{n},N,M))^T,
% \end{equation*}
% where $\mathbf{n}$ is a vector-variate random variable attributed to a multivariate Gaussian distribution $\mathbf{n} \sim  \mathcal{N}(\mathbf{0}, \bm{\Pi})$, $\bm{\Pi} \in \mathbb{PD}_+^{MN\times MN}$ (the set of positive definite matrices of size $MN\times MN$), and ${\rm{resize}}(\cdot, N, M)$ is an operator that resizes $\mathbf{n}$ into an $N\times M$ matrix.\footnote{For example, ${\rm{resize}}([1,2,3,4,5,6]^T,2,3) = \begin{bmatrix}
% 1 & 3 & 5\\
% 2 & 4 & 6
% \end{bmatrix}$.}
% \label{AMGIC_def}
% \end{mydef}

% %\subsection{Privacy Analysis}
% MGM protects the privacy of the   matrix-valued query data by adding perturbation noises with covariance matrix $\bm{\Pi}$. We develop the following  sufficient condition for MGM  to achieve ($\epsilon, \delta$)-differential privacy.







% \section{SMGM: Reducing the Magnitude of Noises}\label{smgm}


% \subsection{Design Ideas and Statistical Backgrounds}
% % We develop SMGM based on MGM. 
% Recall that the sufficient condition in Theorem \ref{thm_multivariate} only applies to the smallest singular value of $\bm{\Pi}$, i.e., $\sigma_{\text{min}}(\bm{\Pi})$. %In practice, we can set $\sigma_{\text{min}}(\bm{\Pi}) = \frac{\Delta_2f^2 \tau(\delta)}{\epsilon^2}$. However, 
% Since $\bm{\Pi}\in\mathbb{PSD}^{MN\times MN}$, to obtain a valid instance of $\bm{\Pi}$, we still need to choose the other $MN-1$ singular values  and the associated singular vectors.  As a consequence, there are infinite number of $\bm{\Pi}$'s in the design space of the additive perturbation noise, which   hinders the success of applying MGM in large scale matrix-valued data queries. Previous studies also suffer the similar problem, e.g.,  \cite{Chanyaswad2018}, and they proposed to narrow down the design space by either involving  a domain expert to determine the singular pairs, or  conducting a Principal Component Analysis on the queried data to learn the  singular pairs. However, their methods will inevitably introduce bias, make their mechanism data-dependent, and compromise the privacy guarantee. 


% To address the above issue,  we are motivated to  develop a new mechanism which still perturbs the query results using ``Gaussian type'' noises but with singular covariance matrix. In other words, the noises are drawn from a singular multivariate Gaussian distribution. As a result, we only need to determine the value of the non-zero singular values of $\bm{\Pi}$ to achieve differential privacy. We will elaborate its privacy guarantee in the next Section.  In general, a multivariate Gaussian distribution with a singular covariance matrix of rank $r$ is defined as follows.


 
% \subsection{The Proposed SMGM Mechanism}

% In order to reduce the design space of $\bm{\Pi}$ as much as possible, we consider $\bm{\Pi}$  as a rank $1$ matrix, denoted as $\bm{\Pi}_S$, whose   only non-zero singular value is $\sigma_{S}$. As a result, we can generate an instance of $\bm{\Pi}_S$ via 
% \begin{equation*}
% \bm{\Pi}_S = \sigma_S \mathbf{v}^T\mathbf{v},
% \label{set_pi}
% \end{equation*}
% where $\mathbf{v}\in\R^{MN\times 1}$ is a norm 1 vector (we will discuss how to generate it later). 
% Since $\bm{\Pi}_S \mathbf{v} = \sigma_s \mathbf{v}$, $(\sigma_S,  \mathbf{v})$ is a singular pair of  $\bm{\Pi}_S$. Thus, according to the disintegration theorem and (\ref{mapping_singular}), if we generate $\mathbf{n}$ via
% \begin{equation}
% z\sim\mathcal{N}(0,1)\in\mathbb{R},\quad \mathbf{n} = \mathbf{v}\sqrt{\sigma_s}z,
% \label{eq:singular_Pi}
% \end{equation}
% then, it is attributed to the singular multivariate Gaussian distribution with covariance matrix $\bm{\Pi}_S$.









% \begin{remark}
% Note that Theorem \ref{thm_DMGM} requires that the elements of $\mathbf{v}$ are randomly generated. If instead, $\mathbf{v}$ is generated in a deterministic manner, then ....
% \end{remark}



% \begin{algorithm}
% \small
% \SetKwInOut{Input}{Input}
% \SetKwInOut{Output}{Output}
% \caption{Workflow of the proposed SMGM mechanism}\label{algo:workflow}
% \Input{Privacy budget $\epsilon$ and $\delta$, and dimension of the matrix-valued query $f(D)$, i.e., $M$ and $N$}
% \Output{$(\epsilon,\delta)$-deferentially private matrix-valued query $\mathbb{SMGM}(f(D))$.}

% $\mathbf{v} \leftarrow \mathbf{0}^{MN\times 1}$, and $z\sim\mathcal{N}(0,1)$.

% \For{$i\in[1,MN]$}{

% $\mathbf{v}_i\sim \mathcal{N}(0,1)$.

% }

% $\mathbf{v} \leftarrow \frac{\mathbf{v}}{||\mathbf{v}||_2}$.

% $\mathbf{n} \leftarrow \mathbf{v}\sqrt{\sigma_s}z$

% $\mathbf{N} \leftarrow \Big(\mathrm{resize}(\mathbf{n},N,M)\Big)^T$. // $\mathbf{U}$ is any orthonormal basis in $\R^P$.

% $\mathbb{SMGM}(f(D)) \leftarrow f(D)+\mathbf{N}$


% \end{algorithm}
















% \subsection{Discussions and Mechanism Application Caveat}\label{sec:mec_discussion}
% It is noteworthy that the proposed SMGM differs from the    Gaussian mechanism and MVG. This is because in the Gaussian mechanism,   elements of $f(D)$ are perturbed by noises drawn i.i.d. from a univariate Gaussian distribution with variance $\sigma_G^2$, and the collection of these noises forms a multivariate Gaussian distribution with a full rank covariance matrix, i.e., $\sigma_G \mathbf{I}\in\mathbb{PSD}^{MN\times MN}$. 



% However, the proposed SMGM uses singular multivariate Gaussian distribution with a rank 1 covariance matrix, i.e.,  $\bm{\Pi}_S$. In later sections, we will theoretically prove that by introducing singularity into the covariance matrix, SMGM can significantly reduce the magnitude of the additive noise, thus  achieving both lower accuracy loss and higher utility stabilities than the Gaussian mechanism and MVG.  


==> sections/waste-of-gaussian.tex <==




\textbf{Comparing R1SMG and Gaussian Mechanism.} From the proof of Theorem \ref{thm_multivariate}, we know %By combing (\ref{eq:diverge_begin}), (\ref{eq:our_goal}), and (\ref{eq:plrv_r1smg}), it is obvious that  $\mathrm{PLRV}$ associated with our proposed R1SMG is 
\begin{equation}\label{eq:plrv_r1smg_expression}
\mathrm{PLRV}^{(\mathbf{s})}_{(R1SMG(\bm{x})||R1SMG(\bm{x}'))} \leq  \frac{1}{2\sigma_*}\frac{4(\Delta_2f)^2}{sin^2(\theta)},
\end{equation}
where $\theta$ is the angle between the noises ($\mathbf{n}$ and $\mathbf{n}'$) used to perturb $f(\bm{x})$ and $f(\bm{x}')$.  
Recall that,    according to (\ref{eq:plrv2}), for the classical  Gaussian Mechanism we have $\mathrm{PLRV}^{(\mathbf{s})}_{(Gauss(\bm{x})||Gauss(\bm{x}'))} = \frac{1}{2\sigma^2} \Big((\Delta_2f)^2 + 2\lambda_1\Delta_2f\Big)$. 
% and  plugging in $\boldsymbol{v}=f(\bm{x})-f(\bm{x}')$, we have
% \begin{equation*} 
% \mathrm{PLRV}_{\mathcal{M}_G,\bm{x},\bm{x}'}  =  \left|\frac{1}{2\sigma^2}\left(||f(\bm{x})-f(\bm{x}')||^2+2\lambda_1 ||f(\bm{x})-f(\bm{x}')||\right)\right|.
% \end{equation*}
Note again $\sigma_*$ in $\mathrm{PLRV}_{\mathcal{M}_{R1SMG},\bm{x},\bm{x}'}$ is the only non-zero singular value of the covariance matrix ($\bm{\Pi}$) of the additive noise introduced by R1SMG, whereas $\sigma^2$ in $\mathrm{PLRV}^{(\mathbf{s})}_{(Gauss(\bm{x})||Gauss(\bm{x}'))}$ is the variance of the noise used in the Gaussian mechanism. 

$\mathrm{PLRV}^{(\mathbf{s})}_{(R1SMG(\bm{x})||R1SMG(\bm{x}'))}$ and $\mathrm{PLRV}^{(\mathbf{s})}_{(Gauss(\bm{x})||Gauss(\bm{x}'))}$ are both quadratic in $\Delta_2f$. The randomness of  $\mathrm{PLRV}^{(\mathbf{s})}_{(Gauss(\bm{x})||Gauss(\bm{x}'))}$ is characterized by $\lambda_1\sim\mathcal{N}(0,\sigma^2)$ (see Section \ref{sec:evidence}), on the other hand, the randomness of  $\mathrm{PLRV}^{(\mathbf{s})}_{(R1SMG(\bm{x})||R1SMG(\bm{x}'))}$ is due the nondeterministic $sin^2(\theta)$. According to the analysis in Remark \ref{remark:converge_pi2}, $sin(\theta)$ will quickly increases from 0 to 1 (at the rate of $\sqrt{M}$) as $M$ increases, which implies that $\mathrm{PLRV}^{(\mathbf{s})}_{(R1SMG(\bm{x})||R1SMG(\bm{x}'))}$ will decrease for any given $\epsilon$, $\delta$, and $\sigma_*$.  

%angle used to perturb $f(\bm{x})$ and $f(\bm{x}')$. 

The above discussion suggests that by leveraging new source of randomness (i.e., the random angle between noises used to perturb query on neighboring databases), the privacy guarantee can be improved. It further implies a viable approach to   improve the classical Gaussian mechanism. In particular, we can arrive at the following conclusion. 

\begin{theorem}\label{claim:gaussian_with_angle}
    A sufficient condition for the classical Gaussian mechanism to achieve $(\epsilon,\delta)$-DP on $f(\bm{x})\in\R^{M}$ is 
    \begin{equation}\label{eq:gaussian_with_angle}
        (M-1)\mathcal{O}(|\ln   \Delta_2f| ) +  \frac{1}{\sigma^2}\frac{2(\Delta_2f)^2}{\psi}\leq \epsilon, 
    \end{equation}
    where   $\psi = \left(\frac{\delta\Gamma(\frac{M-1}{2})}{\sqrt{\pi}\Gamma(\frac{M}{2})}\right)^{\frac{2}{M-2}}$ and   $\Gamma(\cdot)$ is Gamma  function. 
\end{theorem}
\begin{remark}
The proof of 
 Comment \ref{claim:gaussian_with_angle} is discussed in the next section. 
    Note that      one can develop a new theorem for the classical Gaussian mechanism to achieve $(\epsilon,\delta)$-DP based on the results of Comment \ref{claim:gaussian_with_angle} by just replacing  $\mathcal{O}(|\ln   \Delta_2f| )$ in (\ref{eq:gaussian_with_angle}) with  the tail bound of Chi distributed random variable (discussed in the Proof). However, we do not pursue this, as it is not the main contribution of this paper, and it does not break the curse of full rank covariance matrices.
\end{remark}


\textbf{Proof of Comment \ref{claim:gaussian_with_angle} and Discussions.} First, we review the following result (which rephrases Theorem C.1 (a) and (d) on page 742 of  \cite{paolella2018linear}).

\begin{theorem}\textbf{Decomposition of Spherically Symmetric Random Variable \cite{paolella2018linear}.} \label{thm:ss_decomp} For a spherically symmetric distributed random variable  $\mathbf{n}\in\R^M$, one can express it as 
 $\mathbf{n}\stackrel{d}{=}w\mathbf{V}$, where $\stackrel{d}{=}$ means equality in distribution, $w$ is a continuous univariate random variable $\Pr[w\geq0]=1$, and $\mathbf{V}$ (independent of $w$) is uniformly distributed on the unit sphere surface in $\R^M$. Random variable $w$ is usually   referred to as the %generating variate or 
 radial random variable. 
\end{theorem}



For any multivariate Gaussian random variable $\mathbf{n}\sim\mathcal{N}(0,\sigma^2 \mathbf{I}_{M\times M})$, it can be represented as a 
scaled multivariate standard Gaussian random variable, i.e., 
$\mathbf{n} = \sigma \mathbf{z}, \mathbf{z}\sim \mathcal{N}(0,\mathbf{I}_{M\times M})$. Since $\mathcal{N}(0,\mathbf{I}_{M\times M})$ is spherically symmetric, according to Theorem \ref{thm:ss_decomp},  $\mathbf{z}$ can   be decomposed via $\mathbf{z} = ||\mathbf{z}|| \frac{\mathbf{z}}{||\mathbf{z}||}= w \mathbf{h}$. Here $w  \stackrel{\Delta}{=} ||\mathbf{z}||$ is a random variable attributed to the Chi distribution with $M$ degrees of freedom, i.e., $w\sim\chi(M)$, and $\mathbf{h}\stackrel{\Delta}{=}\frac{\mathbf{z}}{||\mathbf{z}||}$ is a random variable sampled from the unite sphere $\mathbb{S}^{M-1}$, i.e., $\mathbf{h}\sim\mathcal{U}(\mathbb{V}_{1,M})$. As a result, we have  %$\mathbf{n} \stackrel{d}{=} \sigma w \mathbf{h}$. 
\begin{equation*}\label{eq:alternative_gaussian}
    \mathbf{n} \stackrel{d}{=} \sigma w \mathbf{h},\  \text{where\ } \mathbf{n}\sim\mathcal{N}(0,\sigma^2 \mathbf{I}_{M\times M}), w\sim\chi(M), \mathbf{h}\sim\mathcal{U}(\mathbb{V}_{1,M}).
\end{equation*}
%(\ref{eq:alternative_gaussian}) is 
as an alternative way to generate the noise for the classical Gaussian mechanism. It  further implies that we can derive a new privacy guarantee for  the Gaussian mechanism as follows. 

Still, we let $\bm{x}$ and $\bm{x}'$ be a pair of neighboring databases. Assume that $\mathbf{n} = \sigma w_1 \mathbf{h}$ and $\mathbf{n}' = \sigma w_2 \mathbf{g}$ ($w_1, w_2\sim\chi(M), \mathbf{h},\mathbf{g}\sim\mathcal{U}(\mathbb{V}_{1,M})$) are the random noises used to perturb $f(\bm{x})$ and $f(\bm{x}')$, respectively.  Then, we can  immediate  have %the following relationships
% obtain  the squared norm of the additive noise, e.g., $\mathbf{n}'$, as 
% \begin{equation*}
%     ||\mathbf{n}'||_2^2 = (\sqrt{\sigma_*} z_2 \mathbf{g})^T\sqrt{\sigma_*} z_2 \mathbf{g} \stackrel{*}=   \sigma_*  z_2^2,
% \end{equation*}
% where $*$ is because $\mathbf{g}\in\mathbb{V}_{1,M}$, thus $\mathbf{g}^T\mathbf{g} =1$.
\begin{equation}\label{eq:mapping_back}
    % \begin{aligned}
    w_1 = \frac{1}{\sigma}\mathbf{h}^T\mathbf{n},\quad
    w_2 = \frac{1}{\sigma}\mathbf{g}^T\mathbf{n}'.
    % \end{aligned}
\end{equation}


By following the     proof of Theorem \ref{thm_multivariate}, with $\mathcal{A}$ given in (\ref{eq:the_set}), we have a new   sufficient condition for the classical Gaussian mechanism to achieve $(\epsilon,\delta)$-DP as 
\begin{small}
\begin{equation}
\begin{aligned}
&\int_{\mathbf{h}\in\mathbb{V}_{1,M}}  \frac{1}{\mathrm{Vol}(\mathbb{V}_{1,M})} 
\int_{\Ss\cap\mathcal{A}} \frac{ \Big(\frac{1}{\sigma}\mathbf{h}^T ( \mathbf{s}  -f(\bm{x}) )\Big)^{M-1} \exp\left\{-\Big(\frac{1}{\sigma}\mathbf{h}^T ( \mathbf{s}  -f(\bm{x}) )\Big)^2/2\right\} }{2^{M/2-1}\Gamma(M/2)}  d \mathbf{s} d \mathbf{h}\\
\leq & e^{\epsilon}\int_{\mathbf{g}\in\mathbb{V}_{1,M}}  \frac{1}{\mathrm{Vol}(\mathbb{V}_{1,M})}
\int_{\Ss\cap\mathcal{A}} \frac{ \Big(\frac{1}{\sigma}\mathbf{g}^T ( \mathbf{s}  -f(\bm{x}') )\Big)^{M-1} \exp\left\{-\Big(\frac{1}{\sigma}\mathbf{g}^T ( \mathbf{s}  -f(\bm{x}') )\Big)^2/2\right\} }{2^{M/2-1}\Gamma(M/2)} d \mathbf{s} d \mathbf{g},
\end{aligned}
\label{eq:ints_gaussian}
\end{equation}
\end{small}
$\forall\mathbf s \in \Ss\cap\mathcal{A}$, where the inner integrand (i.e, integral kernel) on each side of (\ref{eq:ints_gaussian}) is the PDF of Chi distribution $\chi(M)$, and the outer integrand is the PDF provided in (\ref{eq:stiefel_uniform}). Then, one can easily check that it is sufficient to prove 
$\mathrm{PLRV}_{\mathcal{M}_{G\mathrm{new}},\bm{x},\bm{x}'}$ (the new $\mathrm{PLRV}$ of Gaussian mechanism which now involves the randomness of unit vector $\mathbf{h}$ and $\mathbf{g}$) is   upper bounded by $\epsilon$ for 
 all $\mathbf s \in \Ss\cap\mathcal{A}$, i.e.,  $\mathrm{PLRV}_{\mathcal{M}_{G\mathrm{new}},\bm{x},\bm{x}'} \leq \epsilon$. In particular, we have  
 \begin{small}
\begin{equation*}\label{eq:PRLV_derivative}
\begin{aligned}
&\mathrm{PLRV}_{\mathcal{M}_{G\mathrm{new}},\bm{x},\bm{x}'}% \leq \epsilon \\
\\
= &\left|\ln\left(\frac{\Big(\frac{1}{\sigma}\mathbf{h}^T ( \mathbf{s}  -f(\bm{x}) )\Big)^{M-1} \exp\left\{-\Big(\frac{1}{\sigma}\mathbf{h}^T ( \mathbf{s}  -f(\bm{x}) )\Big)^2/2\right\} }{\Big(\frac{1}{\sigma}\mathbf{g}^T ( \mathbf{s}  -f(\bm{x}') )\Big)^{M-1} \exp\left\{-\Big(\frac{1}{\sigma}\mathbf{g}^T ( \mathbf{s}  -f(\bm{x}') )\Big)^2/2\right\} } \right) \right|\\
%\leq \ln e^{\epsilon}\\
 = & \left| (M-1)\ln\left( \frac{\mathbf{h}^T ( \mathbf{s}  -f(\bm{x})}{\mathbf{g}^T ( \mathbf{s}  -f(\bm{x}')} \right) + 
\frac{1}{2\sigma^2}  \left(     \Bigg(  \underbrace{ \mathbf{g}^T (\mathbf{s}-f(\bm{x}')) }_{\rho_1\in \R}  \Bigg)^2  - \Bigg( \underbrace{ \mathbf{h}^T (\mathbf{s}-f(\bm{x})) }_{\rho_2\in \R}\Bigg)^2   \right) \right| \\ %\leq \epsilon\\
\stackrel{(a)}\leq & (M-1)\left|\ln\left( \frac{ ||\mathbf{s}  -f(\bm{x})||}{|| \mathbf{s}  -f(\bm{x}')||} \right) \right|+  \frac{1}{2\sigma^2}\frac{4(\Delta_2f)^2}{\psi} %\leq \epsilon\\
\\
=  & (M-1)\left|\ln\left( \frac{|| \mathbf{s}  -f(\bm{x})' + f(\bm{x})'-f(\bm{x})||}{|| \mathbf{s}  -f(\bm{x}')||} \right)\right| +  \frac{1}{\sigma^2}\frac{2(\Delta_2f)^2}{\psi}\\ % \leq \epsilon, 
\leq  & (M-1)\left|\ln\left( 1+ \frac{ \Delta_2f}{|| \mathbf{s}  -f(\bm{x}')||} \right)\right| +  \frac{1}{\sigma^2}\frac{2(\Delta_2f)^2}{\psi},
% \Leftrightarrow & (M-1)\ln\left( 1+ \frac{ \Delta_2f}{|| \mathbf{s}  -f(\bm{x}')||} \right) +  \frac{1}{2\sigma^2}\frac{(\Delta_2f)^2}{sin^2(\theta)}\leq \epsilon\\
% \Leftrightarrow & (M-1)\mathcal{O}(\ln   \Delta_2f ) +  \frac{1}{2\sigma^2}\frac{(\Delta_2f)^2}{sin^2(\theta)}\leq \epsilon,
\end{aligned}
\end{equation*}
\end{small}
where $(a)$ is achieved by directly using the fact that  $\mathbf{h}$ and $\mathbf{g}$ are unit vectors and the result of Theorem \ref{thm_multivariate}. 

Clearly, a sufficient condition to make $\mathrm{PLRV}_{\mathcal{M}_{G\mathrm{new}},\bm{x},\bm{x}'} \leq \epsilon$  holds is $$(M-1)\left|\ln\left( 1+ \frac{ \Delta_2f}{|| \mathbf{s}  -f(\bm{x}')||} \right)\right| +  \frac{1}{\sigma^2}\frac{2(\Delta_2f)^2}{\psi}\leq \epsilon,$$ where the left part can easily  be upper bounded by applying the tail bound of Chi distributed random variable since  $|| \mathbf{s}  -f(\bm{x}')|| = ||\mathbf{n}'||\sim\chi(M)$.  Yet, we will stop here and write $(M-1)\left|\ln\left( 1+ \frac{ \Delta_2f}{|| \mathbf{s}  -f(\bm{x}')||} \right)\right| = (M-1)\mathcal{O}(|\ln\Delta_2f|)$, which complete proving the conclusion in Comment \ref{claim:gaussian_with_angle}. 

Comparing $\mathrm{PLRV}_{\mathcal{M}_{G\mathrm{new}},\bm{x},\bm{x}'}$ with 
$\mathrm{PLRV}_{\mathcal{M}_{R1SMG},\bm{x},\bm{x}'}$ (in (\ref{eq:plrv_r1smg_expression})), the classical Gaussian mechanism is able to  save at  least $(M-1)\Omega(|\ln\Delta_2f|)$ privacy budgets, should the covariance matrix has rank 1. Here we use $\Omega(|\ln\Delta_2f|)$ to represent a lower bound of $\left|\ln\left( 1+ \frac{ \Delta_2f}{|| \mathbf{s}  -f(\bm{x}')||} \right)\right|$.

 

%falls into $(\frac{\pi}{2}-\theta_0,\frac{\pi}{2}+\theta_0)$

% the intrinsic randomness already
% makes Bagging, a popular ensemble learning framework, differentially private without   additional noise \cite{ijcai-bagging}


% \subsection{Practical Implementation of $r$SMGM}



% Recall that the sufficient condition in Theorem \ref{thm_multivariate} only applies to the smallest nonzero singular value of $\bm{\Pi}$, i.e., $\sigma_{r}(\bm{\Pi})$. %In practice, we can set $\sigma_{\text{min}}(\bm{\Pi}) = \frac{\Delta_2f^2 \tau(\delta)}{\epsilon^2}$. However, 
% To successfully apply $r$SMGM, we need to determine an instance of $\bm{\Pi}$. Since there are infinite number of $\bm{\Pi}\in\mathbb{PSD}^{MN\times MN}$ that satisfies the condition in Theorem \ref{thm_multivariate}, which will lead to an infinite design space. Previous studies also suffer the similar problem, e.g., in the MVG mechanism, the authors proposed to narrow down the design space by either involving  a domain expert to determine the singular pairs, or  conducting a Principal Component Analysis on the queried data to learn the  singular pairs. However, their methods will inevitably introduce bias, and make their mechanism data-dependent.


% To make $r$SMGM dataset independent (i.e., the singular pairs of $\bm{\Pi}$ are not determined by $f(D)$), we propose to generate the required noise samples using Algorithm \ref{algo:rsmgm}.



% \begin{algorithm}
% \small
% \SetKwInOut{Input}{Input}
% \SetKwInOut{Output}{Output}
% \caption{Generate noise samples in $r$SMGM}\label{algo:rsmgm}
% \Input{Dimension of matrix-valued query, i.e, $M$ and $N$, privacy budget $\epsilon$ and $\delta$.} % maintained by the data curator.}
% \Output{Noise samples $\mathbf{n}$ whose covariance matrix is $\bm{\Pi}\in\mathbb{PSD}^{MN\times MN}$ and $Rank(\bm{\Pi})=r$.}% released to the data consumer.}


% Sample $\mathbf{V}_r\sim \mathcal{B}(r,MN;\mathbf{B})\in\mathcal{V}_{r,MN}$.\label{line:Bingham_sample}

% Randomly assign $\sigma_1\geq\sigma_2\geq\cdots\geq \sigma_r = \frac{\Delta_2f^2\omega(\delta,r)}{\epsilon^2}$.\label{line:assignment}

% Synthesize $\bm{\Pi} = \mathbf{V}_r \mathrm{diag}(\sigma_1,\cdots,\sigma_r)   \mathbf{V}_r^T$.

% Sample $\mathbf{n}$ attributed to $f_{\mathbf{x};Rank(\bm{\Pi})=r}$ by applying (\ref{mapping_singular}). % in Definition \ref{def:singular_pdf}.

% \end{algorithm}
% % \begin{equation}
% % \boxed{
% %     \begin{aligned}
% %   \mathrm{Sample}\quad & \mathbf{V}_r\sim \mathcal{B}(r,MN;\mathbf{B})\in\mathcal{V}_{r,MN},\\
% %   \mathrm{Randomly\ assign} \quad & \sigma_1\geq\sigma_2\geq\cdots\geq \sigma_r = \frac{\Delta_2f^2\omega(\delta,r)}{\epsilon^2},\\
% %   \mathrm{Synthesize} \quad & \bm{\Pi} = \mathbf{V}_r \mathrm{diag}(\sigma_1,\cdots,\sigma_r)   \mathbf{V}_r^T.
% %     \end{aligned}
% %     }
% %     \label{eq:rsmgm_procedure}
% % \end{equation}
% In   Algorithm \ref{algo:rsmgm}, $\mathcal{B}(r,MN;\mathbf{B})$ represents the matrix Bingham distribution  with a symmetric parameter matrix $\mathbf{B}$. It takes values on the support of Stiefel Manifold $\mathcal{V}_{r,MN} = \{\mathbf{V}_r\in\R^{MN\times r}:\mathbf{V}_r^T\mathbf{V}_r = \mathbf{I}_{r\times r},r<MN\}$, i.e., $\mathbf{V}_r$ is a set of $r$ orthonormal vectors in $\R^{MN\times 1}$.  The PDF of  $\mathcal{B}(r,MN;\mathbf{B})$ takes the following form 
% \begin{equation}\label{eq:binham_pdf}
% f(\mathbf{V}_r;\mathbf{B}) = \frac{1}{{}_{1}F_{1}(\frac{1}{2}r,\frac{1}{2}MN,\mathbf{B})}\exp\Big(\Tr[\mathbf{V}_r^T\mathbf{B}\mathbf{V}_r]\Big),
% \end{equation}
% where 
% % $\mathbf{V}$ is the desired $N\times k$ matrix with orthonormal columns, and
% ${}_{1}F_{1}(\frac{1}{2}r,\frac{1}{2}MN,\mathbf{B})$ is a confluent
% hypergeometric function (cf. \cite{chikuse2012statistics}, page 33), and $\mathbf{B}$ can be any positive definite symmetric matrix. 


